Realization Theory of Stochastic Jump-Markov Linear Systems

In this paper, we present a complete stochastic realization theory for stochastic jump-linear systems. We present necessary and sufficient conditions for the existence of a realization, along with a characterization of minimality in terms of reachability and observability. We also formulate a realization algorithm and argue that minimality can be checked algorithmically. The main tool for solving the stochastic realization problem for jump-linear systems is the formulation and solution of a stochastic realization problem for a general class of bilinear systems with non-white-noise inputs. The solution to this generalized stochastic bilinear realization problem is based on the theory of formal power series. Stochastic jump-linear systems represent a special case of generalized stochastic bilinear systems.

==> GBS_real_power_series.tex <==
\section{Rational Power Series}
\label{sect:pow}
%In this section, we present several results on formal power series, which will be used for solving a general bilinear filtering/realization problem to be presented in Section \ref{gen:filt}. In turn, the solution to this bilinear filtering/realization problem will yield a solution to the realization problem for stochastic jump-linear systems, as we will show in Sections \ref{sect:GJMLS}--\ref{sect:GJMLS_real:necc}. 
The material and results in Subsections \ref{hscc_pow_basic} and \ref{hscc_pow_stab} can be found in \cite{MP:Phd} and \cite{MPRV:HSCC}, respectively. For more details on the classical theory of rational formal power series, the reader is referred to \cite{Reut:Book,Son:Real,Son:Resp} and the references therein.
 
%\subsection{ Definitions}
%\label{hscc_pow_basic}

Let $\Sigma$ be a finite set. We will refer to $\Sigma$ as the \emph{alphabet}. The elements of $\Sigma$ will be called \emph{letters}, and every finite sequence of letters will be called a  \emph{word} or \emph{string} over $\Sigma$.
 Denote by $\Sigma^{*}$ the set of all words from elements in $\Sigma$. The length
 of a word $w$ is denited by $|w|$.
 %An element $w\in \Sigma^{*}$ of length $|w|=k\geq 0$ is a finite sequence
 %$w=\sigma_{1} \sigma_{2} \cdots \sigma_{k}$ with  $\sigma_{1},\ldots, \sigma_{k} \in \Sigma$.
The empty word is denoted by $\epsilon$ and its length is zero, \ie $|\epsilon|=0$.
Denote by $\Sigma^{+}$ the set of all non-empty words
over $\Sigma$, \ie $\Sigma^{+}=\Sigma^{*}\setminus \{\epsilon\}$.
 The concatenation of two words $v=\nu_{1} \cdots \nu_{m}$ and 
$w=\sigma_{1} \cdots \sigma_{k} \in \Sigma^{*}$
 is the word $vw=\nu_{1} \cdots \nu_{m}\sigma_{1} \cdots \sigma_{k}$.

In the sequel we will use the following lexicographic ordering on $\Sigma^{*}$. 
\begin{Definition}[Lexicographic ordering]
\label{rem:lex} Let  $<$ be an ordering on $\Sigma$ so that $\Sigma=\{\sigma_1,\ldots,\sigma_{|\Sigma|}\}$ with $\sigma_1 < \sigma_2 < \ldots < \sigma_{|\Sigma|}$. We define a lexicographic ordering $\prec$ on $\Sigma^{*}$ as follows. For any $v=\nu_{1} \cdots \nu_{m}$ and $w=\sigma_{1} \cdots \sigma_{k} \in \Sigma^{*}$, $v \prec w$ if either $|v| < |w|$ or $0 < |v|=|w|$, $v \ne w$ and for some $l \le |w|$, $\nu_l < \sigma_l$ with the ordering $<$ on $\Sigma$ an $\nu_i = \sigma_i$ for $i=1,\ldots, l-1$. 
\end{Definition}
Notice that $\prec$ is a complete ordering and that $\Sigma^{*}=\{v_0,v_1,\ldots \}$ with $v_0 \prec v_1 \prec \ldots $. Therefore, we will call the set $\{v_0,v_1,\ldots\}$ an \emph{ordered enumeration} of $\Sigma^*$. Notice also that $v_0 =\epsilon$ and that for all $i \in \mathbb{N}$ and $\sigma \in \Sigma$, we have $\nu_i \prec \nu_i\sigma$. Moreover, denote by $M(N)$ the number of all non-empty words over $\Sigma$ whose length is at most $N$, \ie $M(N)=|\{w \in \Sigma^{+} \mid |w| \le N\}|$. It then follows
that with the lexicographic ordering defined above,  the set $\{v_0,v_1,\ldots,v_{M(N)}\}$ equals to the set of
all words of length at most $M(N)$, including the empty word.

  A \emph{formal power series} $S$ with coefficients in 
  $\mathbb{R}^{p}$ is a map
  \( S: \Sigma^{*} \rightarrow \mathbb{R}^{p} \).
  We will call the values $S(w) \in \mathbb{R}^{p}$, $w \in \Sigma^{*}$, the \emph{coefficients} of
  $S$.
   We will denote by
   $\FPS$ the set of all formal power series
   with coefficients in $\mathbb{R}^{p}$.
    Consider a family of formal power series
    $\Psi=\{ S_{j}  \in \FPS \mid j \in J\}$
    indexed with a finite index set
    $J$. 
    The $\Psi$
    will be called \emph{rational} if 
    there exists an integer $n \in \mathbb{N}$, a matrix
   $C \in \mathbb{R}^{p \times n} $, a 
   collection of matrices 
   $A_{\sigma} \in \mathbb{R}^{n \times n}$
   indexed by $\sigma \in \Sigma$,  and an indexed set 
   $B=\{ B_{j} \in \mathbb{R}^{n} \mid j \in J\}$ 
   of vectors in $\mathbb{R}^{n}$, such that  for each index 
   $j \in J$ and for all sequences 
   $\sigma_{1}, \ldots, \sigma_{k} \in \Sigma$, $k \ge 0$,  
%
  \begin{align}
      S_{j}(\sigma_{1}\sigma_{2} \cdots \sigma_{k})=
      CA_{\sigma_{k}}A_{\sigma_{k-1}} \cdots A_{\sigma_{1}}B_{j}.
  \end{align}
The 4-tuple $R=(\mathbb{R}^{n},\{A_{\sigma}\}_{\sigma \in \Sigma},B,C)$ will be called a \emph{representation} of $\Psi$ and the number $n = \dim R$ will be called the \emph{dimension} of $R$. A representation $R_{min}$ of $\Psi$ will be called \emph{minimal} if all representations $R$ of $\Psi$ satisfy \( \dim R_{min} \le \dim R \). Two representations of $\Psi$, $R=(\mathbb{R}^{n},\{ A_{\sigma} \}_{\sigma \in \Sigma},B,C)$ and $\widetilde{R}=(\mathbb{R}^{n},\{ \widetilde{A}_{\sigma} \}_{\sigma \in \Sigma}, \widetilde{B},\widetilde{C})$, will be called \emph{isomorphic}, if there exists  a nonsingular matrix $T \in \mathbb{R}^{n \times n}$ such that$T\widetilde{A}_{\sigma}=A_{\sigma}T$ for all $\sigma \in \Sigma$, $T\widetilde{B}_{j}=B_{j}$ for all $j \in J$, and $\widetilde{C}=CT$. 

Let $R=(\mathbb{R}^{n},\{A_{\sigma}\}_{\sigma \in \Sigma},B,C)$ be a representation of $\Psi$. In order to characterize whether this representation is reachable and observable, let us define the following short-hand notation
\begin{Notation}
\label{matrix:prod}
   $A_{w} \!\doteq\! A_{\sigma_{k}}A_{\sigma_{k-1}} \!\!\cdots A_{\sigma_{1}}$ for
   $w=\sigma_{1} \cdots \sigma_{k}\in \Sigma^*$ and
   $\sigma_1,\ldots, \sigma_k \in \Sigma$, $k \ge 0$.
The map $A_{\epsilon}$ will be identified with the identity map. 
\end{Notation}|
Recall the ordered enumeration of $\Sigma^*$, $\{v_0,v_1,\ldots\}$,  fix an enumeration  of $J=\{j_1,\ldots,j_K\}$ and let $\widetilde{B}=\begin{bmatrix} B_{j_1} & \cdots & B_{j_K} \end{bmatrix}$.
Define the following matrices.
 %
  \begin{align}
 \label{sect:pow:form1}
 %%W_{R} &= \quad \SPAN\{ A_{w}B_{j} \mid w \in \Sigma^{*}, |w| \le n-1, j \in J\}  \; \\
 W_{R} &= \begin{bmatrix} A_{v_0}\widetilde{B} &, \ldots, & A_{v_{M(n-1)}}\widetilde{B} \end{bmatrix} \\
\label{sect:pow:form1.1}
 %O_{R} &=  \!\!\!\!\bigcap_{w \in \Sigma^{*}, |w| \le n-1} 
%                 \!\!\!\!\!\!\!\!\!\ker CA_{w}.
   O_R &= \begin{bmatrix} (CA_{v_0})^T & \ldots & (CA_{v_{M(n-1)}})^T \end{bmatrix}^T.
  \end{align}
  %
 We will call the representation $R$ \emph{observable} if $\ker O_{R} = \{0\}$ and \emph{reachable} if $\dim R = \Rank W_{R}$.
Observability and reachability of representations can be checked numerically. 
%For instance, one can formulate an algorithm for transforming any 
%representation to a minimal representation of the same
%family of formal power series (see 
%\cite{MP:Phd} and the references therein for details).
Let $\Psi=\{ S_{j} \in \FPS \mid j \in J\}$. We define 
the Hankel-matrix $H_{\Psi}$ of $\Psi$ as  the matrix such that the following holds.
%whose entries are given by  $(H_{\Psi})_{(u,i)(v,j)}= (S_{j}(vu))_{i}$.
The rows of $H_{\Psi}$ are indexed by pairs
$(u,i)$ where $u\in\Sigma^*$ is a word over $\Sigma$ and $i$ is
and integer in $I=\{1,2,\ldots,p \}$. Likewise, the columns of
$H_{\Psi}$ are indexed by pairs $(v,j)$, where
$v\in\Sigma^*$ and $j$ is an element of the index set $J$. 
Thus, the element of $H_{\Psi}$ whose
row index is $(u,i)$ and whose
column index is $(v,j)$ is simply the $i$th row
of the vector $S_{j}(vu)\in\Re^p$, i.e. $(H_{\Psi})_{(u,i)(v,j)}= (S_{j}(vu))_{i}$.
      
      The following result on realization of formal power series can be found in
       \cite{Son:Real,Son:Resp,MP:Phd}.
 \begin{Theorem}[Realization of formal power series]
 \label{sect:form:theo1}
\label{sect:pow:theo1}
    Let $\Psi=\{ S_{j} \in \mathbb{R}^{p}\ll \Sigma^{*} \gg \mid j \in J\}$ be a set of formal power series indexed by $J$.
    Then the following holds.
  \begin{itemize}
  \item[(i) ]
  $\Psi$ is rational $\iff$ $\Rank H_{\Psi} < +\infty$.
  \item[(ii)]
   $R$ is  a minimal representation of $\Psi$ 
   $\iff$ $R$ is reachable and observable $\iff$
   $\dim R=\Rank H_{\Psi}$.
  \item[(iii)] All minimal representations of $\Psi$ are isomorphic.
 % \item[(iv)]
 %  If the rank of the Hankel matrix $H_{\Psi}$ is finite,
 %  \ie $n=\Rank H_{\Psi} < +\infty$, then one can construct a 
 %  representation $R=(\mathbb{R}^{n}, \{A_{\sigma}\}_{\sigma \in \Sigma}, B,C)$ of $\Psi$
 %  using the columns of $H_{\Psi}$ (see
 %  \cite{MP:Phd} for details). 
\end{itemize}    
\end{Theorem}
%Notice that $H_{\Psi}$ is an infinite matrix and hence the construction in 
%part (iv) of Theorem \ref{sect:pow:theo1} is not directly computable. However, 
It is possible to compute a minimal representation of 
$\Psi$ from finitely many data, see \cite{MP:PartReal,Isidori:TAC73} for a detailed
exposition. 
Define he finite matrix $H_{\Psi,M,N}$ as
the finite upper-left block of the infinite Hankel matrix $H_{\Psi}$
obtained by taking all the rows of
$H_{\Psi}$ indexed by words over $\Sigma$ of length at most $M$, and
all the columns of $H_{\Psi}$ indexed by words of length at most $N$.
%If $\Rank H_{\Psi,N,N}=\Rank H_{\Psi}$ holds, then
%there exists an algorithm for computing a minimal representation
%$R_{N}$ of $\Psi$. The algorithm is essentially a generalization
%of the well-known Kalman-Ho algorithm \cite{Ho-Kalman:Allerton65} for linear systems.
%The condition $\Rank H_{\Psi,N,N}=\Rank H_{\Psi}$ holds, if,
%for example, $N$ is chosen to be 
%bigger than the dimension of some representation of $\Psi$.
%In practice, this means that $N$ has to be an upper bound on
%the estimated dimension of a potential representation of $\Psi$.
%In order to present the algorithm, we define the notion of \emph{$r,N$-selection}:
%an \emph{$r,N$-selection} is a pair $(\alpha,beta)$ such that
Consider a pair of finite sets $(\alpha,\beta)$ such that
\begin{enumerate}
\item
$\alpha \subseteq \Sigma^{N} \times \{1,\ldots,p\}$, 
$\beta \subseteq \Sigma^{N} \times J$, $\Sigma^{N}=\{v \in \Sigma^{*} \mid |v| \le N\}$,
\item
 $|\alpha|=|\beta|=r$.
\end{enumerate}
Denote by 
 $H_{\Psi}^{\alpha,\beta}$ be the matrix formed by the intersection of the columns of $H_{\Psi,N,N}$ indexed by elements of $\beta$ with the rows of $H_{\Psi,N,N}$ indexed by the elements of $\alpha$.
Intuitively, $\alpha$ represents a selection of $r$ rows of $H_{\Psi,N,N}$ and
$\beta$ represents a selection of $r$ columns of $H_{\Psi,N,N}$.
We will call the pair
$(\alpha,\beta)$ be an \emph{$r,N$-selection}. 
The proposed algorithm takes as parameter
the matrix $H_{\Psi,N+1,N}$ and an $r,N$-selection $(\alpha,\beta)$. 
%$\alpha=\{(u_1,j_1),\ldots, (u_r,j_r)\}$, $\beta=\{(v_1,j_1),\ldots, (v_r,j_r)\}$.
%Define the matrix
%\[   H_{\Psi,\alpha,\beta}=((S_{j_l}(v_lu_k))_{i_k}))_{l,k=1,\ldots,r} \in \mathbb{R}^{r \times r}.
%\]
%We assume that $r=\Rank H_{\Psi,\alpha,\beta}=\Rank H_{\Psi,N+1,N}$.
\begin{algorithm}
\caption{
\label{alg1} 
 \newline
\textbf{Inputs:} matrix $H_{\Psi,N+1,N}$ and  $r,N$-selection $(\alpha,\beta)$ 
 \newline
\textbf{Output:} representation $\widetilde{R}_N$.
}
\begin{algorithmic}
%%\STATE 
%%   %Let $r=\Rank H_{\Psi,N,N}$ and choose
%%   $j_{1},\ldots, j_{r} \in J$, $i_{1},\ldots, i_{r} \in \{1,\ldots,p\}$,
%%   $v_{1},\ldots, v_{r}, u_{1},\ldots, u_{r} \in \Sigma^{*}$
%%   such that  for all $l=1,\ldots, r$, 
%%   $|v_{l}| \le N$ and $|u_{l}| \le N$, and
%%   the matrix
%%   %%\begin{equation}
%%   \(
%%   T=((S_{j_{k}}(v_{k}u_{l}))_{i_{l}}))_{l,k=1,\ldots, r} \in \mathbb{R}^{r \times r}
%%   %%\end{equation}
%%   \) of $H_{\Psi,N,N}$ is of
%%   rank $r$. %%\ie $\Rank T=r$.
\STATE 
    For each symbol 
    $\sigma \in \Sigma$ let $A_{\sigma} \in \mathbb{R}^{r \times r}$
    be such that %%for each $l=1,\ldots, r$
    \[ A_{\sigma}H_{\Psi,\alpha,\beta}=Z_{\sigma} \]
  \mbox{  where }
  $Z_{\sigma}$ is $r \times r$ matrix with row indices from $\alpha$ and column indices from
  $\beta$ such that its entry indexed by $z \in \alpha$, $(v,j) \in \beta$ equals
  the entry of $H_{\Psi,N,N+1}$ indexed by $(z,(v\sigma,j))$.

  
  %$i$th column of $H_{\Psi,\alpha,\beta}$ corresponds to the column 
  %indexed by $(v,j) \in \beta$, then 
  %the $i$th column of $Z_{\sigma}$ is formed by the column of
  %$H_{\Psi}$ indexed by $(v\sigma,j)$ and the rows which are indexed by elements of $\alpha$,
  %$i=1,\ldots,r$.
\STATE
    Let $B=\{ B_{j} \mid j \in J\}$, where for each 
    index $j \in J$, the vector
    $B_{j} \in \mathbb{R}^{r}$ is formed by those entries of
    the column $(\epsilon,j)$ of $H_{\Psi}$ which are indexed by the elements of $\alpha$.
%%
\STATE
    Let $C \in \mathbb{R}^{p \times r}$ whose $i$th row is the interesection of 
    the row indexed by $(\epsilon,i)$ with the columns of $H_{\Psi}$ indexed by the elements of
    $\beta$, $i=1,2,\ldots,p$.
\STATE Return $\widetilde{R}_N=(\mathbb{R}^{r}, \{A_{\sigma}\}_{\sigma \in \Sigma},B,C)$.
\end{algorithmic}
\end{algorithm}
\begin{Theorem}[\cite{MP:Phd,Son:Real,SontagMod}]
\label{sect:part:theo1}
   If $r=\Rank H_{\Psi,N,N}=\Rank H_{\Psi}$, then 
   there exists an $r,N$-selection $(\alpha,\beta)$ such that
   $\Rank H_{\Psi,\alpha,\beta}=r$ and the 
   the representation
   $\widetilde{R}_{N}$ returned by
   Algorithm \ref{alg1} when applied to $H_{\Psi,N+1,N}$ and $(\alpha,\beta)$
   is minimal representation of $\Psi$.
 Furthermore, if $\Rank H_{\Psi} \le N$, or, equivalently, there exists a representation $R$ of $\Psi$, such that $\dim R \le N$, then
 $\Rank H_{\Psi}=\Rank H_{\Psi,N,N}$, hence 
 $\widetilde{R}_{N}$ is a minimal 
 representation of $\Psi$.
\end{Theorem}
%\subsection{ A Notion of Stability for Formal Power Series}
%\label{hscc_pow_stab}
%%%\input{JMLS_real_stability_power_series}
For our purposes one has to restrict attention to formal power series that are stable in some sense, similarly to the case of linear systems. In this subsection, we consider the notion of square summability for formal power series, and translate the requirement of square summability into algebraic properties of their representations.
Consider a formal power series $S \in \mathbb{R}^{p}\ll \Sigma^{*} \gg$ and define the sequence 
%%%
 \begin{align} 
 L_{n}=\sum_{k=0}^{n} \sum_{\sigma_{1} \in \Sigma} \cdots 
 \sum_{\sigma_{k} \in \Sigma} 
 ||S(\sigma_{1}\sigma_{2}\cdots \sigma_{k})||^{2}_{2} .
 \end{align}
%
where $||\cdot||_{2}$ is the Euclidean norm
in $\mathbb{R}^{p}$. 
The series $S$ will be called \emph{square summable}, if the
limit $\lim_{n \rightarrow +\infty} L_{n}$ exists and it
is finite. The family 
 $\Psi=\{ S_{j} \in \mathbb{R}^{p}\ll \Sigma^{*} \gg \mid j \in J\}$
 will be called \emph{square summable}, if
 for each $j \in J$, the formal power series 
 $S_{j}$ is square summable. 
%We now characterize square summability of a family of formal power series in terms of the stability of its representation. Let $R=(\mathbb{R}^{n}, \{ A_{\sigma} \}_{\sigma \in \Sigma}, B,C)$ be an arbitrary representation of $\Psi=\{ S_{j} \in \mathbb{R}^{p}\ll \Sigma^{*} \gg \mid j \in J\}$ and
and consider the matrix 
 \( \widetilde{A}=\sum_{\sigma \in \Sigma} A_{\sigma}^{T} \otimes A_{\sigma}^{T} \).
  We will call $R$ \emph{stable}, if the matrix
  $\widetilde{A}$ is stable, \ie
  if all
  its eigenvalues $\lambda$ lie inside the unit disk ($|\lambda| < 1$).
  \begin{Theorem}[\cite{MPRV:JMPL}]
  \label{hscc_pow_stab:theo2}
   If $\Psi$ admits a 
   stable representation, then $\Psi$ is square summable.
   If $\Psi$ is square summable, then any minimal representation of $\Psi$ is stable.
  \end{Theorem}
%%   Notice the analogy with the case of linear systems, where the minimal
%%   realization of a stable transfer matrix is also stable. 
%%\begin{proof}[Proof of Theorem \ref{hscc_pow_stab:theo2}]
%%Assume that $\Psi$ has a stable representation $R=(\mathbb{R}^{n}, \{ A_{\sigma}\}_{\sigma\in \Sigma},C,B)$. Then all the eigenvalues of the matrix $\widetilde{A}=\sum_{\sigma \in \Sigma} A_{\sigma}^{T} \otimes A_{\sigma}^T$ are inside the unit circle. One can easily see that the matrix $\widetilde{A}$ is in fact a matrix representation of the linear map $\Z : \Re^{n\times n} \to \Re^{n\times n}$ defined as \[  \Z(V)=\sum_{\sigma \in \Sigma} A_\sigma^TVA_\sigma .\]  This result is obtained by identifying $\Re^{n\times n}$ with $\Re^{n^2}$,  as it is done in \cite[Section 2.1]{CostaBook}. As a consequence, the eigenvalues of $\Z$ and $\widetilde{A}$ coincide. Since the eigenvalues of $\Z$ are inside the unit circle, it follows from \cite[Proposition 2.5]{CostaBook} that for each positive semi-definite matrix $V \ge 0$,  the infinite sum
%%    \(   \sum_{k=0}^{\infty} \|\mathcal{Z}^{k}(V)\|  \)
%%    is convergent. By noticing that
%%    \[ \forall x \in \Re^n ~~ x^T\mathcal{Z}^{k}(V)x \le \| x \|_{2}^2  \cdot \| \Z^{k}(V) \|, \]
%%    we conclude that $\sum_{k=0}^{\infty} x^T\mathcal{Z}^{k}(V)x$
%%   is convergent for all $x$. It can be shown by induction that
%%   %
%%  \begin{equation}
%%   \label{hscc_pow_stab:lemma2:eq2}
%%     \mathcal{Z}^{k}(V) = \sum_{w \in \Sigma^{*}, |w|=k} A_{w}^TVA_{w}.
%%    \end{equation}
%%    %
%%    Thus, letting $V=C^TC$ in $\sum_{k=0}^{\infty} x^T\mathcal{Z}^{k}(V)x$, we conclude that 
%%   \( \sum_{w \in \Sigma^{*}} \|CA_{w}x\|_{2}^{2} \)
%%   is convergent for all $x$. If we set $x=B_j$, $j \in J$,
%%   we then obtain that $\sum_{w \in \Sigma^{*}} \|S_{j}(w) \|_{2}^{2}$ is convergent for all $j \in J$, \ie the family $\Psi$
%%  is square summable.
%%
%%
%%
%%%%Then for some $Q > 0$, the series
%%%%   $\sum_{w \in X^{*}} B_j^TA_{w}^TQA_{w}B_j$  will be
%%%%   convergent for each $j \in J$. There exists a constant
%%%%   $M > 0$, such that for all $x \in \mathbb{R}^n$,
%%%%   \[ x^TC^TCx \le M x^TQx \]
%%%%   and hence 
%%%%   \[ \sum_{w \in X^{*}} ||S_j(w)||_{2}^2 = 
%%%%       \sum_{w \in X^{*}} B_j^TA_{w}^TC^TCA_{w}B_j
%%%%       \le 
%%%%      \sum_{w \in X^{*}} B_j^TA_{w}^TQA_{w}B_j.
%%%%   \]
%%%%   That is, for each $j \in J$,
%%%%   $\sum_{w \in X^{*}} ||S_{j}(w)||_{2}^{2}$ is 
%%%%   convergent and hence $\Psi$ is square summable.
%%
%%Assume now that $\Psi$ is square summable and let $R=(\mathbb{R}^{n}, \{ A_{\sigma}\}_{\sigma \in \Sigma},C,B)$ be a minimal representation of $\Psi$. Also, let $Q=O_{R}^TO_{R} > 0$, where $O_R$ is the observability matrix of $R$, which is full rank because $R$ is observable. 
%%%
%%First we show that
%%%
%%   \begin{equation}
%%   \label{hscc_pow_stab:lemma2:eq11}
%%    \sum_{k=0}^\infty x^T \Z^k(Q) x = \sum_{w \in \Sigma^{*}} x^TA_{w}^TQA_{w}x
%%   \end{equation}  
%%%
%%is convergent for all $x \in \mathbb{R}^{n}$. To see this, notice from the reachability of $R$ that any $x \in \mathbb{R}^{n}$ is a linear combination of vectors of the form $A_vB_j$, $j \in J$, $v \in \Sigma^{*}$. Hence, it is sufficient to prove the convergence of \eqref{hscc_pow_stab:lemma2:eq11} for $x=A_vB_j$. But the latter follow from the fact that \[ \sum_{w\in\Sigma^*}(B_jA_v)^TA_{w}^TQA_wA_vB_j=  \sum_{w\in\Sigma^*} \sum_{i=0}^{M(n-1)} ||S_{j}(vwv_i)||_{2}^{2}\] and that $\sum_{w \in \Sigma^{*}} \|S_{j}(w)\|^2_2$, hence $\sum_{w \in \Sigma^{*}} \sum_{i=0}^{M(n-1)} \|S_{j}(vwv_i)\|_{2}^{2}$ is convergent. Next we show that 
%%%
%%   \begin{equation}
%%    \sum_{k=0}^\infty x^T \Z^k(V) x = \sum_{w \in \Sigma^{*}} x^TA_{w}^TVA_{w}x
%%   \end{equation}  
%%%
%%is convergent for all $x \in \mathbb{R}^{n}$ and for all positive semi-definite $n\times n$ matrices $V \geq 0$. To see this, notice that for all $V \ge 0$   and $Q > 0$, there exists $M > 0$ such that $x^TVx \le M x^TQx$ for all $x \in\mathbb{R}^n$. Indeed, we can choose $M=\frac{\|V\|}{m}$, where $0 < m=\inf_{\|x\|=1} x^TQx$, so that $m\|x\|^2 \le x^TQx$ and hence $x^TVx \le \|x\|^{2}\|V\| \le M x^TQx$. Therefore, for any $V \ge 0$,
%%   \[ 
%%        \sum_{k=0}^\infty x^T\mathcal{Z}^{k}(V)x =
%%     \sum_{w \in \Sigma^{*}} x^TA_{w}^TVA_{w}x \le
%%       M \sum_{w \in \Sigma^{*}} x^TA_{w}^TQA_{w}x = 
%%       M \sum_{k=0}^\infty x^T\mathcal{Z}^{k}(Q)x,
%%    \]
%%%
%%and so $\sum_{k=0}^\infty x^T\mathcal{Z}^{k}(V)x$ is convergent for all $x\in\Re^n$ and $V\geq 0$. This implies that
%%%
%%    \[ \lim_{k \rightarrow \infty} x^T\mathcal{Z}^{k}(V)x = 0
%%    \]
%%%
%%    for all $x \in \mathbb{R}^n$. Therefore, 
%%     $\lim_{k \rightarrow \infty} \mathcal{Z}^{k}(V) = 0$
%%    for all $V \ge 0$, 
%%    which by \cite[Proposition 2.5]{CostaBook} implies
%%    that all the eigenvalues of $\mathcal{Z}$ (and hence
%%    of $\widetilde{A}$) have 
%%    modulus strictly smaller than $1$, \ie $R$ is stable.
%%
%%%%   Next, we show that if $R$ is stable, then
%%%%   for some $Q > 0$,
%%%%   $\sum_{w \in X^{*}} x^TA_{w}^TQA_{w}x$ is convergent.
%%%%   Indeed, 
%%%%   from \cite[Proposition 2.5]{CostaBook}, it follows that
%%%%   if all the eigenvalues of $\mathcal{Z}$ lie inside the unit
%%%%    circle, and hence $R$ is stable, then 
%%%%    Hence, if \eqref{hscc_pow_stab:lemma2:eq1} is convergent
%%%%    for $V=I$, then so is
%%%%    $\sum_{k=0}^{T} x^T\mathcal{Z}^{k}(I)x$ for all
%%%%    $x$. By \eqref{hscc_pow_stab:lemma2:eq2} it then
%%%%    follows that for $Q=I$, 
%%%%    $\sum_{w \in X^{*}} x^TA_{w}^TQA_{w}x$ converges for
%%%%    all $x$.
%%    
%%     
%%
%%
%%%%     Let $\widetilde{A}_{R}=\widetilde{A}$.
%%%%   
%%%%   \texttt{ $\widetilde{A}$ stable $\implies$
%%%%            $\sum_{w \in X^{*}} ||A_{w}x||_{2}^{2} < +\infty$} 
%%%%	    
%%%%     Assume that $\widetilde{A}$ is stable.
%%%%     Consider the following linear maps
%%%%     \( D: \mathbb{R}^{n^{2}} \cong 
%%%%        \mathbb{R}^{n} \times \mathbb{R}^{n} \rightarrow 
%%%%	\mathbb{R}
%%%%     \)	
%%%%     \( D(e_{i} \otimes e_{j})=\left\{\begin{array}{rl}
%%%%                                      1 & \mbox{ if } i=j \\
%%%%				      0 & \mbox{ otherwise }
%%%%				\end{array}\right.      
%%%%        \), where
%%%%     It is easy to see that $D(x \otimes y)=x^{T}y$.
%%%%     It is clear that we can view $D$ as a vector 
%%%%     in $\mathbb{R}^{1 \times n^{2}}$
%%%%     Let
%%%%     \( \widetilde{D}=\frac{1}{d}\begin{bmatrix} D & \cdots &
%%%%         D \end{bmatrix} \in \mathbb{R}^{1 \times n^{2}d}
%%%%     \).	 
%%%%     Notice that $A_{z} \otimes A_{z}(x \otimes y)=A_{z}x \otimes A_{z}y$.
%%%%     Hence, by induction it follows that for all $k \ge 0$,
%%%%     \[ \widetilde{A}^{k}\begin{bmatrix} x \otimes y \\
%%%%                      x \otimes y \\ \cdots  \\ x \otimes y 
%%%%		      \end{bmatrix} =
%%%%              \begin{bmatrix} 
%%%%	         \sum_{z_{1},\ldots, z_{k} \in X}
%%%%		  (A_{z_{k}}A_{z_{k-1}} \cdots A_{z_{1}}x) \otimes
%%%%		  (A_{z_{k}}A_{z_{k-1}} \cdots A_{z_{1}}y)
%%%%               \\
%%%%	         \sum_{z_{1},\ldots, z_{k} \in X}
%%%%		  (A_{z_{k}}A_{z_{k-1}} \cdots A_{z_{1}}x) \otimes
%%%%		  (A_{z_{k}}A_{z_{k-1}} \cdots A_{z_{1}}y)
%%%%	       \\	  
%%%%	       \vdots \\
%%%%	         \sum_{z_{1},\ldots, z_{k} \in X}
%%%%		  (A_{z_{k}}A_{z_{k-1}} \cdots A_{z_{1}}x) \otimes
%%%%		  (A_{z_{k}}A_{z_{k-1}} \cdots A_{z_{1}}y)
%%%%             \end{bmatrix}
%%%%      \]	     
%%%%   Hence, with 
%%%%   \( \widetilde{x}=
%%%%     \begin{bmatrix} x \otimes x \\ x \otimes x \\
%%%%             \vdots \\ x \otimes x
%%%%        \end{bmatrix}
%%%%   \)
%%%%   Hence it holds that
%%%%   \[ \widetilde{D}\widetilde{A}^{k}x=
%%%%	\sum_{v \in X^{*}, |v|=k} (A_{v}x)^{T}(A_{v}x)
%%%%	=\sum_{v \in X^{*}, |v|=k}
%%%%	 ||A_{v}x||_{2}^{2}
%%%%   \]
%%%%   which implies that 
%%%%   \( \sum_{w \in X^{*}} || A_{v}x ||_{2}^{2} =
%%%%      \sum_{k=0}^{+\infty} \widetilde{D}\widetilde{A}\widetilde{x}
%%%%    \).
%%%%  Hence, if $\widetilde{A}$ is stable, the series
%%%%  $\sum_{w \in X^{*}} ||A_{w}x||_{2}^{2}$ is convergent.
%%%%
%%%%  \texttt{ $\sum_{w \in X^{*}} ||A_{w}x||^{2}_{2} <+\infty$
%%%%     for all $x \in X$ $\implies$ $\widetilde{A}$ is stable} \\
%%%%     
%%%%    We will show that for all $z \in \mathbb{R}^{n^{2}d}$,
%%%%     \[ \lim_{k \rightarrow +\infty} \widetilde{A}^{k}z = 0 \]
%%%%     It follows from the classical theory that if the equality
%%%%     above holds for all $z \in \mathbb{R}^{n^{2}d}$, then
%%%%     $\widetilde{A}$ is stable.
%%%%     Let $z=(z_{1}^{T},\ldots, z_{d}^{T}) \in \mathbb{R}^{n^{2}d}$,
%%%%     $z_{1},\ldots, z_{d} \in \mathbb{R}^{n^{2}} \cong \mathbb{R}^{n} \otimes \mathbb{R}^{n}$.
%%%%     Assume that 
%%%%     $z_{i}=x_{i} \otimes y_{i}$, $x_{i},y_{i} \in \mathbb{R}^{n}$,
%%%%     $i=1,\ldots,d$.
%%%%     It is easy to see that 
%%%%     \[ \widetilde{A}^{k+1}z =
%%%%        \sum_{i=1}^{d}
%%%%        \sum_{v \in X^{*}, |v|=k}
%%%%	 A_{v}A_{z_{i}}x_{i} \otimes A_{v}A_{z_{i}}y_{i}
%%%%     \]	 
%%%%     Notice that $(x \otimes y)^{T}(z \otimes h)=(x^{T}y)(z^{T}h)$.
%%%%     Hence,
%%%%     \[ ||\widetilde{A}^{k+1}z||_{2}^{2}=
%%%%        \sum_{i,j=1}^{d} \sum_{v,w \in X^{*}, |w|=|v|=k}
%%%%	 (x_{i}^{T}A_{z_{i}}A_{v}^{T}A_{w}A_{z_{j}}x_{j})
%%%% (y_{i}^{T}A_{z_{i}}A_{v}^{T}A_{w}A_{z_{j}}y_{j})
%%%%     \] 
%%%%
%%%%     But for all $s,h \in \mathbb{R}^{n}$, 
%%%%     \[ |s^{T}A_{v}^{T}A_{w}h| \le
%%%%        ||A_{v}s||^{2} ||A_{w}h||_{2}
%%%%     \]	
%%%%     Hence, 
%%%%     \[
%%%%       \begin{split} 
%%%%        & ||\widetilde{A}^{k+1}z||_{2}^{2} \le
%%%%	\sum_{i,j=1}^{d} \sum_{w,v \in X^{*}, |w|=|v|=k }
%%%%	  (||A_{v}A_{z_{i}}x_{i}||_{2} \cdot ||A_{w}A_{z_{j}}x_{j}||_{2} \cdot
%%%%	  ||A_{v}A_{z_{i}}y_{i}||_{2} \cdot ||A_{w}A_{z_{j}}y_{j}||_{2} \le \\
%%%%         & \le (\sum_{i=1}^{d} \sum_{w \in X^{*}, |w|=k}
%%%%	       ||A_{w}A_{z_{i}}x_{i} ||_{2} \cdot ||A_{w}A_{z_{i}}y_{i}||_{2})^{2}
%%%%	 \end{split}      
%%%%     \]
%%%%     But  
%%%%     \[ ||A_{w}A_{z_{i}}x_{i}||_{2}\cdot ||A_{w}A_{z_{i}}y_{i}||_{2}  \le
%%%%        \frac{1}{2} (||A_{w}A_{z_{i}}x_{i}||^{2}_{2}+||A_{w}A_{z_{i}}y_{i}||_{2}^{2})
%%%%     \]
%%%%     Hence	
%%%%     \[ \sum_{w \in X^{*}, |w|=k}
%%%%         ||A_{w}A_{z_{i}}x_{i}||_{2}||A_{w}A_{z_{i}}y_{i}||_{2} \le
%%%%	  \frac{1}{2}
%%%%	  (\sum_{w \in X^{*}, |w|=k}
%%%%	    ||A_{w}A_{z_{i}}x_{i}||^{2}_{2}) + \frac{1}{2}
%%%%	    (\sum_{w \in X^{*}, |w|=k} ||A_{w}A_{z_{i}}y_{i}||_{2}^{2})
%%%%      \]
%%%%      Since $\sum_{w \in X^{*}} ||A_{w}x||_{2}^{2}$ converges
%%%%      for all $x \in \mathbb{R}^{n}$, it follows that
%%%%      \[ \lim_{k \rightarrow +\infty} \sum_{w \in X^{*}, |w|=k}
%%%%         ||A_{w}x||_{2}^{2} = 0 
%%%%       \]
%%%%       for all $x \in \mathbb{R}^{n}$.Hence we get that
%%%%       for all $z \in \mathbb{R}^{n^{2}d}$
%%%%       \[ \lim_{k \rightarrow +\infty}
%%%%           ||\widetilde{A}^{k}z||_{2}^{2} = 0
%%%%        \]	   
%%%%  That is, $\widetilde{A}$ is stable.
%%%%
%%%%  \texttt{ $R$ is stable $\implies$ $\Psi$ is square summable} \\
%%%%    If $R$ is stable, then for all $j \in J$,
%%%%    \[ \sum_{w \in X^{*}} ||S_{j}(w)||_{2}^{2} =
%%%%       \sum_{w \in X^{*}} ||CA_{w}B_{j}||^{2}_{2} \le
%%%%       ||C||_{2}^{2} ||A_{w}B_{j}||^{2}_{2} < +\infty
%%%%    \]   
%%%%   That is, $S_{j}$ is square summable for all $j \in J$. 
%%  %\end{proof}
%%%%  \begin{proof}[Proof of Theorem \ref{hscc_pow_stab:theo2}]
%%%%   It is clear that if all minimal representations are stable and
%%%%   $\Psi$ is rational, then there exists at least one 
%%%%   stable minimal representation, which by Lemma \ref{hscc_pow_stab:lemma2} implies that $\Psi$ is square summable.
%%%%   
%%%%   It is left to prove the only if part of the theorem.
%%%%   Assume that $\Psi$ is square summable.
%%%%   Let $R=(\mathbb{R}^{n},\{A_{z}\}_{z \in X}, C,B)$ be a 
%%%%   minimal representation of $\Psi$. 
%%%%   We will show that 
%%%%   \[ \sum_{v \in X^{*}} ||A_{v}x||_{2}^{2} < +\infty \]
%%%%   for
%%%%   all $x \in \mathbb{R}^{n}$. By Lemma \ref{hscc_pow_stab:lemma2}
%%%%   it already implies that $R$ is stable.
%%%%      Let $\mathbb{N} \ni N \le n$.
%%%%      Consider the set 
%%%%      \[ W_{N}=\{ f: X^{\le N} \rightarrow \mathbb{R}^{p} \mid \mbox{ f is an arbitrary function } \} \]
%%%%      where 
%%%%      $X^{\le N}=\{ w \in X^{*} \mid |w| \le N\}$.
%%%%      Notice that $W_{N}$ is a vector space with pointwise
%%%%      addition and multiplication and it is isomorphic as
%%%%     a vector space to 
%%%%      $\mathbb{R}^{d(\sum_{j=0}^{N} d^{j})}$.
%%%%     Define the map 
%%%%    \( O_{N}: \mathbb{R}^{n^{2}d} \rightarrow W_{N} \) 
%%%%    as follows. For each $z \in \mathbb{R}^{n}$,
%%%%    \[  O_{N}(z)(w)=CA_{w}x \]
%%%%    From the observability of $R$ it follows that 
%%%%    $\Rank O_{N}=n$, hence the map
%%%%    \[ ||. ||_{N}: \mathbb{R}^{n} \ni x \mapsto ||Q_{N}x||_{N,p,2}
%%%%    \]
%%%%    defines a norm on $\mathbb{R}^{n}$, where
%%%%    $||.||_{N,p,2}$ is the Eucledian norm on 
%%%%    $W_{N} \cong \mathbb{R}^{p(\sum_{j=0}^{N} d^{j})}$.
%%%%    That is, 
%%%%    \[ ||f||_{N,p,2}^{2}=\sum_{w \in X^{*}, |w| \le N} ||f(w)||_{2}^{2} 
%%%%    \]
%%%%    Since $R$ is reachable, it follows that for each $x \in \mathbb{R}^{n}$, 
%%%%    there exists $\alpha_{i} \in \mathbb{R}, w_{i} \in X^{*}, j_{i} \in J$, $i=1,\ldots, M$ such that
%%%%    $x=\sum_{i=1}^{M} \alpha_{i}A_{w_{i}}B_{j_{i}}$.
%%%%    Hence, 
%%%%    \[ \sum_{v \in X^{*}} ||A_{v}x||_{N}^{2}=
%%%%       \sum_{i=1}^{M} |\alpha_{i}| 
%%%%       \sum_{v \in X^{*}} ||O_{N}A_{v}A_{w_{i}}B_{j_{i}}||_{N,p,2}^{2}
%%%%    \]
%%%%    But 
%%%%    \[ ||O_{N}A_{v}A_{w_{i}}B_{j_{i}}||_{N,p,2}^{2}=
%%         \sum_{w \in X^{*}, |w| \le N} 
%%	  ||CA_{w}A_{v}A_{w_{i}}B_{j_{i}}||_{2}^{2}=
%%	  \sum_{w \in X^{*}, |w| \le N}
%%	   ||S_{j_{i}}(wvw_{i})||^{2}_{2}
%%    \]
%%    Hence
%%    \[ \sum_{v \in X^{*}} 
%%        ||A_{v}x||_{N}^{2} =
%%	\sum_{i=1}^{M} |\alpha_{i}| 
%%	\sum_{w \in X^{*}, |w| \le N}
%%	\sum_{v \in X^{*}}
%%	 ||S_{j_{i}}(wvw_{i})||^{2}_{2} < +\infty
%%     \] \ie
%%     $\sum_{v \in X^{*}} ||A_{v}x||_{N}^{2}$ is convergent.
%%     But all norms on $\mathbb{R}^{n}$ are equivalent, hence,
%%     there exists $K >0$ such that
%%     $||x||_{2}^{2} \le K ||x||_{N}^{2}$ for all $x \in \mathbb{R}^{n}$
%%     which implies that 
%%     $\sum_{v \in X^{*}} ||A_{v}x||_{2}^{2}$ is convergent.
%%   For each $w \in Q^{*}$, let 
%%%%   \[ \hat{A}_{w}=\begin{bmatrix}
%%%%                   A_{w} \otimes A_{w} & 0 & \cdots & 0 \\
%%%%		   0   & A_{w} \otimes A_{w} & \cdots & 0 \\
%%%%		   \vdots & \vdots & \vdots & \vdots \\
%%%%		   0      &    0 & 0 & A_{w} \otimes A_{w}
%%%%		   \end{bmatrix} 
%%%%		   \in \mathbb{R}^{n^{2}d \times n^{2}d}
%%%%  \]		   
%%%%    Using the notation above, we will argue that 
%%%%    for all $x \otimes y$, the sequence
%%%%    \( s_{k}=
%%%%       |\widetilde{D}\hat{A}_{w}\widetilde{A}^{k}
%%%%       \begin{bmatrix} x \otimes y \\ x \otimes y \\
%%%%                       \vdots \\ x \otimes y
%%%%       \end{bmatrix}|
%%%%     \)  
%%%%     converges to $0$.
%%%%     Indeed, by  the inequality
%%%%     $|<x,y>| \le \frac{1}{2}(||x||^{2} + ||y||^{2})$, we get
%%%%     that
%%%%     \[ s_{k}=\sum_{v \in X^{*}, |v|=k}
%%%%            |(CA_{w}A_{v}x)^{T}(CA_{w}A_{v}y|
%%%%	    \le
%%%%	    0.5(\sum_{v \in X^{*}, |v|=k}
%%%%	     ||CA_{w}A_{v}x)||_{2}^{2}) + 
%%%%	     0.5 (\sum_{v \in X^{*}, |v|=k}
%%%%	       ||CA_{w}A_{v}x)||_{2}^{2})
%%%%     \]	       
%%%%     Since $R$ is minimal, it is reachable, hence
%%%%     there exists $\alpha_{s,i}$, $w_{s,i} \in X^{*}$, 
%%%%     $j_{s,i} \in J$, $i=1,\ldots, N$ such that
%%%%     $s=\sum_{i=1}^{N} \alpha_{s,i} A_{w_{s,i}}B_{j_{s,i}}$
%%%%     for $s=x,y$.
%%%%     Hence, for $s=x,y$,
%%%%     \( \sum_{v \in X^{*}} ||CA_{w}A_{v}s||_{2}^{2}=
%%%%        \sum_{i=1}^{N} \alpha_{s,i} \sum_{v \in X^{*}}
%%%%	  ||S_{j_{s,i}}(wvw_{s,i})||_{2}^{2}
%%%%     \)	  
%%%%     By square summability of $\Psi$ the series above are
%%%%     convergent, hence
%%%%     $\sum_{v \in X^{*}, |v|=k} ||CA_{w}A_{v}s||_{2}^{2}$
%%%%     tends to $0$ as $k \rightarrow +\infty$. Hence,
%%%%     $\lim_{k \rightarrow +\infty} s_{k}=0$.
%%%%
%%%%     That is, for all $z \in \mathbb{R}^{n^{2}} \cong \mathbb{R}^{n} \otimes \mathbb{R}^{n}$,
%%%%     \( \lim_{k \rightarrow +\infty}
%%%%         |\widetilde{D}\hat{A}_{w}\widetilde{A}^{k}\widetilde{z}| = 0
%%%%      \)
%%%%      where $\widetilde{z}=(z^{T},z^{T}, \ldots, z^{T})^{T} \in \mathbb{R}^{n^{2}d}$.
%%%%
%%%%      If $v=(v_{1}^{T},\ldots, v_{d}^{T})^{T} \in \mathbb{R}^{n^{2}d}$, 
%%%%      $v_{i} \in \mathbb{R}^{n^{2}}$, $i=1,\ldots, d$, then
%%%%      $\widetilde{A}v=(s^{T},s^{T},\ldots, s^{T})^{T})$,
%%%%      where $s=\sum_{i=1}^{d} (A_{z_{i}} \otimes A_{z_{i}})v$.
%%%%      Hence, we get that for all $v \in \mathbb{R}^{n^{2}d}$,
%%%%      \( \lim_{k \rightarrow +\infty}
%%%%         |\widetilde{D}\hat{A_{w}}\widetilde{A}^{k}v| =0
%%%%      \).	 
%%%%
%%%%      Consider the set $W_{N}=\{ f: X^{\le N} \rightarrow \mathbb{R}^{d} \mid \mbox{ f is an arbitrary function } \}$, where 
%%%%      $X^{\le N}=\{ w \in X^{*} \mid |w| \le N\}$.
%%%%      Notice that $W_{N}$ is a vector space with pointwise
%%%%      addition and multiplication and it is isomorphic as
%%%%      a vector space to 
%%%%      $\mathbb{R}^{d(\sum_{j=0}^{N} d^{j})}$.
%%%%      Define the map 
%%%%    \( O_{N}: \mathbb{R}^{n^{2}d} \rightarrow W_{N} \) 
%%%%    as follows. For each $z=(z_{1}^{T},\ldots, z_{d}^{T}) \in \mathbb{R}^{n^{2}d}$, $z_{i} \in \mathbb{R}^{n^{2}}$,$i=1,\ldots,d$,
%%%%    let
%%%%    \[ O_{N}(z)(w)=\frac{1}{d}
%%%%                \begin{bmatrix} 
%%%%		 D(A_{w} \otimes A_{w})z_{1} \\
%%%%		 D(A_{w} \otimes A_{w})z_{2} \\
%%%%		 \vdots \\
%%%%		 D(A_{w} \otimes A_{w})z_{d} \\
%%%%		 \end{bmatrix}
%%%%    \]
%%%%    Then it is easy to see that $O_{N}$ is a linear map.
%%%%    Define 
%%\end{proof}


==> JMLS_real_GJMLS_real.tex <==
\section{Realization of Generalized Jump Markov Linear Systems with Fully Observed Discrete State}
\label{sect:GJMLS_real}

%Recall the notion of \emph{realization} for linear stochastic systems \cite{Caines1}.
In this section we will address the realization probelm for fully
observed GJMLSs. That it throughout the section we restrict attention to GJMLS
such  that $o$ is identity, i.e. 
$\lambda(t)=\btheta(t)$ and hence the discrete state can be observed.
For ease of notation, in the sequel we will keep the discrete state process $\btheta$ fixed and whenever we speak of a GJMLS realization of the process $\tilde\y$, we will always mean a GJMLS of $\tilde\y$ with discrete state process $\btheta$.
More precisely, let $\widetilde{\y}(t)$ be a stochastic process taking values in 
$\mathbb{R}^{p}$.
\begin{Definition}[Realization by GJMLS]
The GJMLS $H$ with discrete state process $\btheta$ 
is said a \emph{realization} of $\widetilde{\y}$
if the continuous output process $\y$ of $H$ is equals to $\widetilde{\y}$.
We call a realization $H$ of $(\widetilde{\y},\widetilde{\lambda})$
\emph{minimal}, whenever $\dim H \le \dim H'$ for all JMLSs $H'$
that are %%a weak or square-mean
realizations of $\widetilde{\y}$.
\end{Definition}
This section will be devoted to the solution of the following realization problem
for GJMLSs with fully observed discrete states.
\begin{Problem}[Realization problem for generalized bilinear systems]
 Given a process $\widetilde{\y}(t)$ and find conditions for existence of a
 GJMLS which is a realization of $\widetilde{\y}(t)$ and charecterize minimality
 of GJMLS realizations of $\widetilde{\y}(t)$.
\end{Problem}






 In this subsection, we will formulate a similar concept for GJMLS with fully observed discrete state, \ie $\o(t) = \btheta(t)$. Section \ref{sect:GJMLS_problem_form} defines the realization problem for GJMLS with fully observed discrete states. 
%%Section \ref{real:necc} presents necessary conditions for the existence of a realization of JMLS with partially measured discrete states. 
Section \ref{real:suff} presents necessary and sufficient conditions for the existence of a realization of GJMLS with fully measured discrete state.
Section \ref{real:min} presents a characterization of minimality.


\subsection{GJMLS and \GBS}
 We begin by associating a generalized bilinear system $\BS_{H}$ with a GBJMLS $H$S.
 Let the alphabet $\Sigma$ be the set of pairs of discrete states, \ie $\Sigma=Q \times Q$. For each letter $(q_{1},q_{2}) \in \Sigma$ let the input processes of $B$ be defined as
%
  \begin{equation}
  \bu_{(q_{1},q_{2})}(t)=
     \chi(\btheta(t+1)=q_{2},\btheta(t)=q_{1}). 
     \end{equation}
%
Define $p_{(q_1,q_2)}=p_{q_1,q_2}$. Notice that Assumption \ref{input:assumptions} holds
with $\alpha_{\sigma}=1$ for all $\sigma \in \Sigma$. 
 We define the
   set of admissible sequences $L$ (see Assumption~\ref{gen:filt:ass1:cond1}) as 
  \begin{equation} 
  \label{real:suff:admiss1}
    L=\{ w=(q_{1},q_{2})(q_{2},q_{3})\cdots (q_{k-1},q_{k}) \mid   k \ge 0, q_{1},q_{2},\ldots, q_{k} \in Q \}.
  \end{equation}
 Notice that if $w=\sigma_1\sigma_2 \cdots \sigma_k \notin L$,
then $\bu_{\sigma_1}(t-k)\cdots \bu_{\sigma_k}(t)=0$.

\begin{Definition}[\GBS\ associated with a GJMLS]
  Assume that $H$ is a GJLS of the form (\ref{stoch_jump_lin:geq1}) and $H$ satisfies 
  Assumptions
  \ref{Assumption0}--\ref{Assumption2}. 
  We will define the \GBS\ 
  $\BS_{H}$, referred to as
  the \emph{\GBS\ associated with $H$} as follows.
  \begin{equation}
   \label{real:gjmls_repr}
     \BS \left \{\begin{split}
      \widetilde{\x}(t+1)&=\sum_{\sigma \in \Sigma} (A_{\sigma}\widetilde{\x}(t)+
       \widetilde{K}_{\sigma}\widetilde{\v(t)})\bu_{\sigma}(t) \\
      \y(t)&=C\widetilde{\x}(t)+D\widetilde{\v}(t),
     \end{split}\right.
     \end{equation}
  %such that $R_{H}$  is a representation of 
  %$\Psi_{\widetilde{\y}}$.
 % The construction goes as follows. Let
  %\begin{equation}
  %%\label{real:gjmls_repr}
  %R_{H}=(\mathbb{R}^{n}, \{ A_{(q_1,q_2)} \}_{(q_1,q_{2}) \in \Sigma}, C, B), 
 % \end{equation}
  where the parameters are defined as follows.

  \textbf{ State $\widetilde{\x}(t)$ of $\BS_{H}$ } \\
   $\widetilde{\x}(t)=\begin{bmatrix} \x^T(t)\chi(\btheta(t)=1), & \ldots, & \x^{T}(t)\btheta(t)=d) \end{bmatrix}^T \in \mathbb{R}^{n}$, $n=n_1+\cdots+n_d$.

 \textbf{ Noise $\widetilde{\v}(t)$ of $\BS_H$} \\
   $\widetilde{\x}(t)=\begin{bmatrix} \v^T(t)\chi(\btheta(t)=1), & \ldots, & \v^{T}(t)\btheta(t)=d) \end{bmatrix}^T \in \mathbb{R}^{dm}$.
     
  \textbf{ Matrices $A_{(q_1,q_2)}$. } \\
   Let
    $n=n_{1}+n_{2}+\cdots +n_{d}$ and
    for each $q_1,q_{2}$ let $A_{q_2,q_1}$ be the 
    $n \times n$ matrix 
    \begin{equation*}
    A_{(q_2,q_1)}=\begin{bmatrix}
                 \delta_{(1,1),(q_1,q_2)}M_{1,1} &
		  \cdots & \delta_{(1,d),(q_1,q_2)}M_{1,d} \\
		  \vdots & \vdots  \vdots \\
		 \delta_{(d,1),(q_1,q_2)}M_{d,1} & \cdots
		 & \delta_{(d,d),(q_1,q_2)}M_{d,d}
		 \end{bmatrix}
    \end{equation*}
    where $\delta_{(i,j),(k,l)}=1$ if $k=i$ and $j=l$ and $\delta_{(i,j),(k,l)}=0$ otherwise.
    That is, all the entries of $A_{q_2,q_1}$ are
    zero except the $n_{q_1} \times n_{q_2}$ block 
    indexed by row indices
    $i \in [n_1+\cdots + n_{q_1-1}+1,n_{1}+\cdots +n_{q_1}]$
    and by column indices
    $j \in [n_1+\cdots + n_{q_2-1}+1,n_{1}+\cdots+n_{q_2}]$,
    which equals $p_{q_1,q_2}M_{q_1,q_2}$.
 

\textbf{The matrix $\widetilde{K}_{q_1,q_2}$} \\
 The $n \times md$ matrix $\widetilde{K}_{q_1,q_2}$ is defined as
 \begin{equation*}
    K_{(q_2,q_1)}=\begin{bmatrix}
                 \delta_{(1,1),(q_1,q_2)}K_{1,1} &
		  \cdots & \delta_{(1,d),(q_1,q_2)}K_{1,d} \\
		  \vdots & \vdots  \vdots \\
		 \delta_{(d,1),(q_1,q_2)}K_{d,1} & \cdots
		 & \delta_{(d,d),(q_1,q_2)}K_{d,d}
		 \end{bmatrix}
    \end{equation*}
    where $\delta_{(i,j),(k,l)}=1$ if $k=i$ and $j=l$ and 
   $\delta_{(i,j),(k,l)}=0$ otherwise.


 \textbf{Matrix $C$.}  \\
    The $p \times n$ matrix $C$ is defined by
    \begin{equation*}
     C=\begin{bmatrix} C_{1} & C_{2} & \cdots & C_{d}
     \end{bmatrix}
    \end{equation*}

\textbf{Matrix $D$} \\
    The $p \times md$ matrix $D$ is defined by
    \begin{equation*}
     D=\begin{bmatrix} D_{1} & D_{2} & \cdots & D_{d}
     \end{bmatrix}
    \end{equation*}

%% \textbf{ Initial states $B$. } 
%%    The family $B=\{ B_{(i,(q_2,q_1))} \mid q_1,q_2 \in Q, i=1,\ldots, p\}$ is defined as follows.
%%    For each $q_1,q_2 \in Q$, $i=1,\ldots, p$,
%%    $B_{(i,(q_2,q_1))}$ is the $ith$ column of
%%    the $n \times p$ matrix 
%%    \begin{equation*}
%%    \begin{bmatrix}  \delta_{1,q_1}G^{T}_{q_2,q_1} & 
%%     \delta_{2,q_1}G^{T}_{q_2,q_1} & \cdots & 
%%     \delta_{d,q_1}G^{T}_{q_2,q_1}
%%    \end{bmatrix}^{T},
%%    \end{equation*}
%%    where  $\delta_{i,j}=1$ if $i=j$ and 
%%    $\delta_{i,j}=0$ if $i \ne j$, and
%%  %%  $G_{q_2,q_1}=E[\x(t)\y^{T}(t-1)\chi(\btheta(t+1)=q_1,\btheta(t)=q_2)]$.
%%    %%\( \delta_{i,j}=\left\{\begin{array}{rl} 
%%    %%            1 & i=j \\
%%    %%		0 & i \ne j
%%    %%		\end{array}\right.
%%    %%\)		
%%   \[ G_{q_2,q_1}=(p_{q_1,q_2}M_{q_1,q_2}P_{q_1}+B_{q_1,q_2}Q_{q_1,q_2}D_{q_1})C_{q_1}^{T}, \]
%%where $Q_{q_1,q_2}=E[\v(t)\v^{T}(t)\chi(\btheta(t+1)=q_2,\btheta(t)=q_1)]$ and
%%$P_{q_2} \in \mathbb{R}^{n_{q_2} \times n_{q_2}}$ 
%%is defined by
%%(\ref{stoch_jump_lin:eq2}).
%%where $G_{q_1,q_2}=pP_q$.
\end{Definition}
\begin{Lemma}
\label{new:stoch_jump_lin:gbs}
 The output process of $H$ and $\BS_{H}$ coincide. If $H$ satisfies
 Assumptions \ref{Assumption0}--\ref{Assumption2}, then $\BS_H$ satisfies Assumption \ref{gbs:def}.
\end{Lemma}
\begin{proof}[Proof of Lemma \ref{new:stoch_jump_lin:gbs}]
\end{proof}
We can reverse the construction above, by associating with every 
\GBS\ $\BS$ a GJMLS $H$.
\begin{Definition}[GJMLS associated with \GBS]
 Let $\BS$ be a \GBS\ of the form \eqref{gen:filt:bil:def}. Define the \emph{GJMLS $H_{\BS}$ associated with $\BS$} as follows.
\begin{equation}
  H_{\BS}: \left \{
  \begin{split}
   \hat{\x}(t+1)&=M_{\btheta(t+1),\btheta(t)}\hat{\x}(t)+
                 \widetilde{K}_{\btheta(t+1),\btheta(t)}\hat{v}(t)  \\
   \widetilde{\y}&=C_{\btheta(t)}\hat{\x}(t) + D_{\btheta(t)}\hat{v}(t), 		 
  \end{split}		 
  \right.
  \end{equation}
%
  where 
%
\begin{enumerate}
\item 
 \textit{Continuous state-spaces. }
  For each $q \in Q$ define 
  $\mathcal{X}_{q} \subseteq  \mathbb{R}^{n}$ 
  as the subspace spanned
  by all the elements
  belonging to $\IM A_{(q_{1},q)}A_{w}K_{\sigma}$ and
  $\IM K_{(q_{1},q)}$ for all
  $q_{1} \in Q$, $w \in \Sigma^{+}$, $\sigma \in \Sigma$,
  $i=1,\ldots, p$. Then identify the elements of $\mathcal{X}_{q}$
  with the elements of $\mathbb{R}^{n_q}$, where $n_{q}=\dim \mathcal{X}_{q}$.
  %
\item  
\textit{State process.} 
The continuous state process $\hat{\x}(t)$ of the GJMLS is  obtained from the continuous state $\x(t)$ of the generelizad bilinear system \ref{gen:filt:eq2} by viewing it as an element of $\mathcal{X}_{\btheta(t)}$ and identifying it with the corresponding vector in $\mathbb{R}^{n_{q}}$ for $q=\btheta(t)$.
%
\item  
\textit{System matrices.} 
For each $q_1,q_2 \in Q$ the matrix $M_{q_{1},q_{2}} \in \mathbb{R}^{n_{q_{2}} \times n_{q_1}}$ is the matrix associated with the linear map 
%
\begin{equation}
\mathcal{X}_{q_{1}} \ni x \mapsto 
     A_{q_{1},q_{2}}x \in  \mathcal{X}_{q_{2}} .
\end{equation}
%
For each $q \in Q$ the matrix $C_{q} \in \mathbb{R}^{p \times n_{q}}$ is the matrix associated with the linear map $\mathcal{X}_{q} \ni x \mapsto Cx \in \mathbb{R}^{p}$, \ie 
$C_{q}$ is the restriction of $C$ to $\mathcal{X}_{q}$.
%
\item 
\textit{Noice process. } 
The noise  process $\hat{\v}(t)$ equals the noise process $\v(t)$ of $\BS$.
%%  \begin{equation}
%%   \begin{split}
%%     \e(t) =\widetilde{\y}(t)-E_{l}[\widetilde{\y}(t) \mid &
%%         \{ \widetilde{\y}(t-k)\chi(\btheta(t-k)=q_{1})\cdots \\
%%	    & \chi(\btheta(t)=q_{k}) \mid 
%%	    q_{1},\ldots, q_{k} \in Q, k \ge 0\}]. 
%%   \end{split}	    
%%  \end{equation}
%%  That is, $\e(t)$ is the difference between
%%  $\widetilde{\y}(t)$ and its projection onto the subspace
%%  formed by the predictor variables 
%%  $\widetilde{\y}(t-k)\chi(\btheta(t-k)=q_{1}) \cdots \chi(\btheta(t)=q_{k})$, 
%%  $k \ge 0$, $q_{1},\ldots, q_{k} \in Q$.
%
\item 
\textit{Noise gain $\widetilde{K}_{(q_1,q_2)}$ and $\widetilde{D}_{q}$ } 
 Set $\widetilde{K}_{(q_1,q_2)}=K_{(q_1,q_2)}$ where the columns of $K_{(q_1,q_2)}$
 are viewed as elements of $\mathcal{X}_q$. Let $D_{q}=D$ for all $q \in Q$.
 

%%Let the matrices $B_{q_1,q_2}$ be defined as follows.
%%Each vector $B_{(i,(q_1,q_2))}$ is an element of $\mathcal{X}_{q_2}$ 
%%and hence can be identified uniquely with a vector in $\mathbb{R}^{n_{q_2}}$.
%%%
%%With this identification let  
%%%$B_{q_{1},q_{2}}$ be the $n_{q_{2}} \times p$ matrix 
%%%
%%\begin{equation}  
%% B_{q_1,q_2}=
%% \begin{bmatrix} 
%% B_{(1,(q_1,q_2))}, & B_{(2,(q_1,q_2))}, & \cdots , & B_{(p,(q_1,q_2))}
%%  \end{bmatrix}  \in \Re^{n_{q_2}\times p}.
%% \end{equation}
%%Let $T_{(q_1,q_{2}),(q_1,q_2)}$ be the self covariance of $\widetilde{\y}(t)\chi(\btheta(t)=q_1,\btheta(t+1)=q_2)$, \ie
%%%
%%\begin{equation} 
%%T_{(q_1,q_2),(q_1,q_2)} =
%%E[\widetilde{\y}(t)\widetilde{\y}^{T}(t)\chi(\btheta(t)=q_1,\btheta(t+1)=q_2)] \in\Re^{p\times p}.
%%\end{equation}
%%%
%%Moreover, let $P_{q_1,q_{2}}$ be the self covariance of $\hat{\x}(t)\chi(\btheta(t)=q_1,\btheta(t+1)=q_2)$, \ie
%%\begin{equation}
%%P_{q_{1},q_{2}}=E[\hat{\x}(t)\hat{\x}^{T}(t)\chi(\btheta(t)=q_1,\btheta(t+1)=q_2)]
%%     \in \mathbb{R}^{n_{q_1} \times n_{q_1}}.
%%\end{equation}
%%%
%%The matrix $K_{q_{1},q_{2}} \in \mathbb{R}^{n_{q_{2}} \times p}$ is defined as 
%%  \begin{equation}
%%  \begin{split}
%%  K_{q_{1},q_{2}}&=(B_{q_{1},q_{2}} - \frac{1}{p_{q_{1},q_2}}
%%      M_{q_{1},q_{2}}P_{q_1,q_2}C_{q_1}^{T}) 
%%       (T_{(q_1,q_2),(q_1,q_2)}- p_{q_1,q_2} C_{q_1}P_{q_1,q_2}C_{q_1}^{T})^{-1}
%%  \end{split}    
%%  \end{equation}
%%  %
\end{enumerate} 
\end{Definition}
\begin{Lemma}
\label{new:stoch_jump_lin:gbs1}
 If $\BS$ is a realization of $\widetilde{\y}$ and $\BS$ satisfies
 Assumptions \ref{gbs:def}, then $H_{\BS}$ is also a 
realization of $\widetilde{\y}$ and $H_{\BS}$ satisfies Assumptions \ref{}--\ref{}.
\end{Lemma}
\begin{proof}[Proof of Lemma \ref{new:stoch_jump_lin:gbs1}]
\end{proof}
 



%%Under assumptions \ref{Assumption0}--\ref{Assumption1.5}, we obtain the following result, which is based on the well-known criteria for mean-square stability of jump-linear systems from \cite{CostaBook}.
%%  
%%  \begin{Lemma}
%%  \label{stoch_jump_stab:lemma1}
%%   If Assumption \ref{Assumption0}--\ref{Assumption1.5} hold, then 
%%   there exists a unique collection of
%%   $n_{q}\times n_{q}$ matrices $P_{q}$ with
%%   $q \in Q$, such that $P_{q}$ satisfy
%%    \begin{equation}
%% \label{stoch_jump_lin:eq2}
%% P_{q}=\sum_{s \in Q} 
%%                     p_{q,s}M_{s,q}P_{s}M_{s,q}^{T}+B_{s,q}Q_{s,q}B_{s,q}^{T}, %%p_{q,s}\pi_{s},
%%  \end{equation}
%%  where $Q_{q,s}=E[\v(t)\v(t)^{T}\chi(\btheta(t+1)=q, \btheta(t)=s)]$.
%%  \end{Lemma}
%% \begin{proof}[Proof of Lemma \ref{stoch_jump_stab:lemma1}]
%%  From Assumption \ref{Assumption0} it follows that
%%  \[
%%   \begin{split}
%%    & E[\v(t)\v^T(t)\chi(\btheta(t+1)=q, \btheta(t)=s)]= 
%%    E[E[\v(t)\v^T(t)\chi(\btheta(t+1)=q, \btheta(t)=s)\mid \mathcal{D}_t]]=\\
%%   & = E[E[\btheta(t+1)=q)\mid \mathcal{D}_t]E[\v(t)\v(t)^T\mid \mathcal{D}_t]]
%%   \end{split}
%%  \]
%%  Note that
%%\[ 
%%  \begin{split}
%%   & \chi(\btheta(t)=r)E[\chi(\btheta(t+1)=q)\mid \mathcal{D}_t]=\\
%%  & \chi(\btheta=r)E[\chi(\btheta(t+1)=q\mid \btheta(t)]=p_{q,r}\chi(\btheta(t)=r)
%% \end{split},
%% \]  due the the Markov propert if $\btheta(t)$.
%% Hence, we get that
%% \[
%%   \begin{split}
%%    & E[\v(t)\v^T(t)\chi(\btheta(t+1)=q, \btheta(t)=s)]=
%%    p_{q,s}E[E[\v(t)\v^T(t)\mid \mathcal{D}_t]\chi(\btheta(t)=s)]=\\
%%   & p_{q,s}E[E[\v(t)\v^T(t)\chi(\btheta(t)=s)\mid \mathcal{D}_t]]=p_{q,s}E[\v(t)\v^T(t)\chi(\btheta(t)=s)].
%%   \end{split}
%%  \]
%% By Assumption \ref{Assumption0}, $E[\v(t)\v^T(t)\chi(\btheta(t)=s)]$ is independent of $t$ and hence $Q_{q,s}$ does
%%  not depend on time. From the definition of $Q_{q,s}$
%%  it follows that that $Q_{q,s}$ is positive semi-definite.
%%
%%
%%  As the next step, define the linear map
%%  $\Z_{d}: (\mathbb{R}^{n \times n})^{d} \rightarrow (\mathbb{R}^{n \times n})^{d})$ defined as follows;
%%  \[ \Z_d((P_1,\ldots,P_d))=(V_1,\ldots, V_d) \]
%%  where for all $q=1,\ldots,d$,
%%  \[ V_q=\sum_{r \in Q} M_{r,q}P_rM_{r,q}^Tp_{q,r}. \]
%%  From \cite{CostaBook} it follows that
%%  $\widetilde{M}$ is just the matrix representation of
%%  $\Z_d$ in the basis defined in \cite[Section 2.1]{CostaBook}.
%%  Hence, $\Z_d$ is stable in the sense of \cite[Section 2.1]{CostaBook}.
%%  Notice that $\mathcal{Z}$ is a positive map, hence
%%  by \cite[Proposition 2.6]{CostaBook} the equation 
%%  \(  V=\Z_d(V)+S \)
%%  has a unique positive-definite solution for any tuple
%%  $S=(S_1,\ldots,S_d)$ of positive definite matrices.
%%  Define $S_q=\sum_{r \in Q} B_{r,q}Q_{r,q}B_{r,q}^T$ for
%%  each $q \in Q$ and set $S=(S_1,\ldots,S_d)$. From the
%%  discussion above it then follows that
%%  there exists a unique solution $V=(P_1,\ldots,P_d)$ such 
%%  that $P_1,\ldots,P_d$ are positive semi-definites and
%%  \( V=\Z_d(V)+S \). The latter is just a different way to
%%  write  \eqref{stoch_jump_lin:eq2}.
%%    
%%
%%
%% \end{proof}
%%Let $\chi$ denote the indicator function, \ie $\chi(A)=1$ if the event $A$ is true, and 
%%  $\chi(A)=0$ otherwise. We will also assume the following.
%%    
%%\begin{Lemma}
%%\label{stoch_jump_stab:lemma2}
%% If Assumption \ref{Assumption2} holds, then 
%%   $E[\x(t)\x(t)^{T}\chi(\btheta(t)=q)]=P_{q}$,
%%   for all $q \in  Q$,
%%   $t \in \mathbb{Z}$.
%%   Here $\{P_q\}_{q \in Q}$ is the unique solution to 
%%   \eqref{stoch_jump_lin:eq2}.
%%\end{Lemma}
%%\begin{proof}[Proof of Lemma \ref{stoch_jump_stab:lemma2}]
%%  A simple calculation reveals that
%%  \[ 
%%    \begin{split}
%%     & E[\x(t+1)\x^T(t+1)\chi(\btheta(t+1)=q)]=
%%     E[M_{\theta(t+1),\theta(t)}\x(t)\x^T(t)M^T_{\theta(t+1),\theta(t)}\chi(\btheta(t+1)=q)]     +   \\
%%      & E[M_{\theta(t+1),\theta(t)}\x(t)\v^T(t)B^T_{\theta(t+1),\theta(t)}\chi(\btheta(t+1)=q)]     +  
%%      E[B_{\theta(t+1),\theta(t)}\v(t)\x^T(t)M^T_{\theta(t+1),\theta(t)}\chi(\btheta(t+1_=q)]     +  \\
%%     & E[B_{\theta(t+1),\theta(t)}\v(t)\v^T(t)M^T_{\theta(t+1),\theta(t)}\chi(\btheta(t+1)=q)]    
%%   \end{split}
%%  \]
%% Notice that 
%% \[ E[M_{\theta(t+1),\theta(t)}\x(t)\x^T(t)M^T_{\theta(t+1),\theta(t)}\chi(\btheta(t+1)=q)]=\sum_{r \in Q} M_{q,r}E[\x(t)\x^T(t)\chi(\btheta(t)=r,\btheta(t+1)=qi)]M_{q,r}^T \]
%%  \[ E[B_{\theta(t+1),\theta(t)}\v(t)\x^T(t)M^T_{\theta(t+1),\theta(t)}\chi(\btheta(t+1)=q)]=\sum_{r \in Q} B_{q,r}E[\v(t)\x^T(t)\chi(\btheta(t)=r,\btheta(t+1)=q)]M_{q,r}^T \]
%%  \[ E[B_{\theta(t+1),\theta(t)}\v(t)\v^T(t)M^T_{\theta(t+1),\theta(t)}\chi(\btheta(t+1)=q)]=\sum_{r \in Q} B_{q,r}E[\v(t)\v^T(t)\chi(\btheta(t)=r,\btheta(t+1)=q)]B_{q,r}^T \]
%%
%% 
%% Recall from the proof of Lemma 
%% \ref{stoch_jump_stab:lemma1} that
%% $E[\chi(\btheta(t+1)=q)\mathcal{D}_t]\chi(\btheta(t)=r)=p_{q,r}\chi(\btheta(t)=q)$.
%% Notice that 
%% Using this and
%% Assumption \ref{Assumption0}, Part \ref{Assumption0:part2},
%% \[ 
%%   \begin{split}
%%    & E[\x(t)\x^T(t)\chi(\btheta(t)=r,\btheta(t+1)=q]=
%%    E[E[\x(t)\x^T(t)\chi(\btheta(t)=r,\btheta(t+1)=q\mid \mathcal{D}_t]]= \\
%%   & =E[E[\x(t)\x^T(t)\mid \mathcal{D}_t]\chi(\btheta(t)=r)
%%      E[\chi(\btheta(t+1)=q)\mathcal{D}_t]]=
%%    p_{q,r}E[\x(t)\x^T(t)\chi(\btheta(t)=r)]
%%  \end{split}
%% \]
%%  By using
%% Assumption \ref{Assumption0}, Part \ref{Assumption0:part2}
%% and Part \ref{Assumption0:part3},
%% and taking conditional expectations with respect
%% of $\mathcal{D}_t$, we obtain
%% \[
%%   \begin{split}
%%    & E[\v(t)\x^T(t)\chi(\btheta(t)=r,\btheta(t+1)=q)]= 
%%    E[E[\v(t)\x^T(t)\chi(\btheta(t)=r,\btheta(t+1)=q)\mid \mathcal{D}_t]]=\\
%%  & = E[E[\v(t)\x^T(t) \mid \mathcal{D}_t]\chi(\btheta(t)=r)E[\chi(\btheta(t+1)=q)\mathcal{D}_t]=0
%%   \end{split}
%%  \]
%%%  Finally, using the same arguments as above,
%%  %\[
%%  %   E[\v(t)\v^T(t)\chi(\btheta(t)=r,\btheta(t+1)=q)]=
%%  %   E[E[\v(t)\v^T(t)\chi(\btheta(t)=r,\btheta(t+1)=q)\mid \mathcal{D}_t]]=E[\v(t)\v^T(t)\chi(\btheta(t)=r)]p_{q,r}
%%  %\]
%%  Combining all the equalities above, and
%%  recalling that $Q_{q,r}= E[\v(t)\v^T(t)\chi(\btheta(t)=r,\btheta(t+1)=q)]$, we obtain
%% \[
%%    E[\x(t+1)\x^T(t+1)\chi(\btheta(t+1)=q)]=
%%    \sum_{r \in Q} (p_{q,r}M_{q,r}E[\x(t)\x^T(t)\chi(\btheta(t+1)=r)]M_{r,q}^T+B_{q,r}Q_{q,r}B_{q,r}^T
%%  \]
%% Since $E[\x(t+1)\x^T(t+1)\chi(\btheta(t+1)=q)]=E[\x(t)\x^T(t)\chi(\btheta(t)=q)]$ for all $t$,  it then follows that
%% $\{ E[\x(t)\x^T(t)\chi(\btheta(t)=q)]\}_{q \in Q}$ is 
%% a solution to \eqref{stoch_jump_lin:eq2}.
%% But by Lemma \ref{stoch_jump_stab:lemma1} the
%% equation \eqref{stoch_jump_lin:eq2} has a unique solution,
%% hence $P_q=E[\x(t)\x^T(t)\chi(\btheta(t)=q)]$.
%%
%%     
%%   
%%  
%% 
%%
%%\end{proof}
Assumptions \ref{Assumption1} and \ref{Assumption2}
are necessary in order to make the continuous state process $\x(t)$ and
the output process $\y(t)$ wide-sense stationary.
%%\subsection{The Realization Problem for GJMLS with Fully Observed Discrete State}
%%\label{sect:GJMLS_problem_form}
%%
%%Let $\widetilde{\y}$ be a zero-mean wide-sense stationary process taking values in $\mathbb{R}^{p}$.
%%%
%%Let $\btheta$ be a Markov-process taking values in $Q=\{1,\ldots,d\}$.
%%%
%%Let $H$ be a GJMLS of the form \eqref{stoch_jump_lin:geq1}, with discrete state process $\btheta$ and output process $\y$, satisfying Assumptions \ref{Assumption0}-\ref{Assumption2}. 
%%%
%%\begin{Definition}[Realization by GJMLS]
%%The GJMLS $H$ is said to be a \emph{square-mean realization} or simply a \emph{realization} of $\widetilde{\y}$ with discrete state process $\btheta$, if the continuous output process $\y$ of $H$ is equals to $\widetilde{\y}$ with probablity $1$.
%% %that is, for any 
%%%time instant $k \in \mathbb{Z}$, $E[(\widetilde{\y}(k)-\y(k))^{T}(\widetilde{\y}(k)-\y(k))]=0$.
%% \end{Definition}
%%For ease of notation, in the sequel we will keep the discrete state process $\btheta$ fixed and whenever we speak of a GJMLS realization of the process $\tilde\y$, we will always mean a GJMLS of $\tilde\y$ with discrete state process $\btheta$.
%%As in the case of linear systems, it is possible for several GJMLS to realize a given process $\tilde\y$. Therefore, we are interested in finding a realization of $\tilde \y$ that is minimal in some sense. We define the notion of a minimal %(weak or square-mean) 
%%realization by a GJLS system as follows.
%%%
%%\begin{Definition}[Minimal Realization by a GJMLS]
%%The \emph{dimension} of a GJMLS $H$ with discrete state process $\btheta$ taking values on $Q=\{1,2,\dots,d\}$ is defined as
%%%
%%\begin{equation} 
%%\dim H =n_{1}+n_{2}+\cdots+n_{d},
%%\end{equation}
%%where $n_i$ is the dimension of the continuous state space associated with discrete state $q$, \ie $n_q = \dim \mathcal{X}_{q}$, for $q\in Q$.
%%%
%%We call a realization $H$ of $\widetilde{\y}$
%%\emph{minimal}, whenever $\dim H \le \dim H'$ for all JMLSs $H'$ 
%%that are %%a weak or square-mean 
%%realizations of $\widetilde{\y}$.
%%\end{Definition}
%%
%%\begin{Remark}
%%Notice that two GJLSs can have the same dimension even if the dimensions of the individual continuous components are completely different.
%%\end{Remark}
%%
%%\textbf{Comment more on this definition, why is good, why is bad}

%%\subsection{Existence of a Realization by a GJMLS with Fully Observed
%% Discrete States}
%%\label{real:suff}
%%
%%In this section, we present necessary and sufficient conditions for the existence of a realization of the output process $\widetilde{\y}$ by a GJMLS with discrete state process $\btheta$. Our results are based on the solution to the Generalized Bilinear Realization Problem presented in Section \ref{gen:filt}. The construction proceeds by associating a generalized bilinear system $B$ to the processes $\tilde\y$ and $\btheta$ and building a formal power series associated with the covariance sequence of the generalized bilinear system. Under certain assumptions, the existence of a GJMLS realization of $\tilde\y$ will be shown to be equivalent to rationality of this formal power series.

 %% From Subsection \ref{real:nec} we know that if
  %%$\widetilde{\y}$ has a realization by a GJMLS $\Sigma$,
  %%then the series $\Psi_{\widetilde{\y},\widetilde{\o}}$
  %%is rational. However, this is only a necessary
  %%condition. 
  
%%We begin by associating a generalized bilinear system $B$ to the given processes $\tilde \y$ and $\btheta$. Let the alphabet $\Sigma$ of $B$ be the set of pairs of discrete states, \ie $\Sigma=Q \times Q$. For each letter $(q_{1},q_{2}) \in \Sigma$ let the input processes of $B$ be defined as
%%%
%%  \begin{equation}
%%  \bu_{(q_{1},q_{2})}(t)=
%%     \chi(\btheta(t+1)=q_{2},\btheta(t)=q_{1}). 
%%     \end{equation}
%%%
%%For each nonempty word $w=\sigma_{1}\cdots \sigma_{k}\in \Sigma^+$, where $\sigma_{1},\ldots, \sigma_{k} \in \Sigma$,  define the regressor variables as in \eqref{gen:filt:eqzdef}, except that the output $\y$ is replaced by the given process $\tilde\y$, \ie
%%   %
%%   \begin{equation}
%%   \z_{w}(t)=\widetilde{\y}(t-k)\bu_{\sigma_{1}}(t-k+1)\cdots \bu_{\sigma_{k}}(t-1). 
%%   \end{equation}
%%  %
%Notice that if $w$ is not of the form $w=(q_{1},q_{2})(q_{2},q_{3})\cdots (q_{k-1},q_{k})$, for $k \ge 0$ and $q_{1},\ldots, q_{k}\in Q$, then
%   $\z_{w}(t)=0$.
%
Notice that if $w\in L$ is an admissible sequence of the form $w=(q_{0},q_{1})(q_{1},q_{2})\cdots (q_{k-1},q_{k})$, then  the covariance $\Lambda_{w} = E[\widetilde{\y}(t)\z_{w}(t)]$ can be written as
%
   \begin{equation}
   \label{real:eq1}
    \Lambda_{w}=E[\widetilde{\y}(t+k)\widetilde{\y}(t)\chi(\btheta(t+i)=q_i, i=0,\ldots, k)].
  \end{equation} 
% 
As in \eqref{gen:filt:pow1}, the sequence of covariances $\Lambda_w$ can be associated with a family of formal power series
%
\( \Psi_{\widetilde{\y}}=\{ S_{(i,\sigma)} \in \FPS
   \mid \sigma \in Q \times Q, i=1,\ldots, p\}
  \),  
%
where  $S_{i,\sigma}(w)$ is the $i$th column of $\Lambda_w$. We will denote this family by $\Psi_{\widetilde{\y}}$ in order to emphasize its dependence on $\widetilde{\y}$.

In order to show that $\Psi_{\widetilde{\y}}$ is well-defined, we
need to assume that Assumption \ref{gen:filt:ass1:cond0} holds.
  
In order to be able to find necessary and sufficient conditions
for the existence of a GJMLS realization, we need to 
make a number of assumptions on $\widetilde{\y}$ and $\btheta$.
Most of these assumptions are also necessary
conditions for the existence of a GJMLS realization.
 
\begin{Assumption}
[Conditional independence of $\widetilde{\y}$ and $\btheta$]
\label{real:suff:ass1.1}
For each $t \in \mathbb{Z}$, the collection of random variables
$\{ \widetilde{\y}(t-l), l \ge 0\} $ and $\{\btheta(t+l) \mid l > 0 \}$ are 
conditionally independent given $\{ \btheta(t-l) \mid l \ge 0 \}$.
\end{Assumption}
%%   This implies that for each sequence $q_{1},\ldots, q_{k} \in Q$
%%   \begin{equation}
%%   \label{real:suff:eq1}
%%   \begin{split}
%%    E[\widetilde{\y}(t)\chi(\btheta(t)=q_{1})
%%      \chi(\btheta(t+1)=q_{2}) \\
%%       \cdots \chi(\btheta(t+k)=q_{k})]= \\
%%    E[\widetilde{\y}(t)\chi(\btheta(t)=q_{1}) \cdots \\
%%      \cdots \chi(\btheta(t+k-1)=q_{k})]p_{q_{k},q_{k-1}}
%%   \end{split}   
%%   \end{equation}
%%   
%% \item 
 
\begin{Assumption}[Stability of $\Psi_{\widetilde{\y}}$]
\label{real:suff:ass1.2}
The familly of formal power series $\Psi_{\widetilde{\y}}$ is square summable.
\end{Assumption}
 
\begin{Assumption}[Ergodicity and strong connectedness of $\btheta$]
 \label{real:suff:ass1.3}
   The Markov process $\btheta$ is stationary, ergodic and
   for each $q_{1},q_{2}$ the transition probability  
    $p_{q_{1},q_{2}} > 0$ is nonzero.
\end{Assumption}
\begin{Assumption}[Full-rank predictor space]
\label{real:suff:ass1.5}
The innovation process $\e(t)=\widetilde{\y}(t) - E_{l}[\widetilde{\y}(t)\mid \{ \z_{w}(t) \mid w \in \Sigma^{+}\} ]$ has the full-rank property, \ie it satisfies Assumption \ref{gen:filt:full_rank} in Section \ref{gen:filt}.
 \end{Assumption}


In the sequel we will use the following notation.

\begin{Notation}[Matrix products]
 We define the following notation for the products of 
  matrices $M_{q_1,q_2} \in \mathbb{R}^{n_{q_1} \times n_{q_2}}$.
For any admissible word $w=(q_1,q_2)\cdots (q_{k-1},q_k) \in L$,
where $k > 2$ and $q_1,\ldots, q_k \in Q$, 
let
\begin{equation}
M_{w}=M_{q_{k-1},q_k}M_{q_{k-2},q_{k-1}}\cdots
   M_{q_1,q_2} \in \Re^{n_{q_k}\times n_{q_1}}
\end{equation}
If $w=\epsilon$, then $M_{\epsilon}$ is an identity matrix,
dimension of which depends on the context it is used in.
If $w \notin L$, then $M_{w}$ denotes the zero matrix.
\end{Notation}
\begin{Notation}[Products of transition probabilities]
 For each admissible word $w=(q_1,q_2)\cdots (q_{k-1},q_k) \in L$,
where $k > 1$ and $q_1,\ldots, q_k \in Q$, let 
  \[ p_w=p_{q_k,q_{k-1}}p_{q_{k-1},q_{k-2}}\cdots p_{q_2,q_1} \]
 If $w \notin L$, then let $p_w=0$. If $w=\epsilon$,
 the set $p_{w}=1$.
\end{Notation}

It is easy to see that the following holds.
  \begin{Lemma}[Wide-sense statonarity]
  \label{real:necc_lemma0}
   If $\widetilde{\y}$ is realizable by a GJLS $H$, then
   $\widetilde{\y}(t)$ is zero mean and
   for any  $w=(q_1,q_2)v \Sigma^{+}$, $v \in \Sigma^{*}$,
   $(q_1,q_2) \in \Sigma=Q \times Q$,
   \begin{equation}
   \label{real:necc_lemma0:eq1}
   \begin{split}
     %& E[\widetilde{\y}(t)\z^T_{w}(t)]=C_{q_2}(p_{q_2,q_1}M_{q_2,q_1}P_{q_1}+B_{q_1,q_2}Q_{q_2,q_1}D_{q_1})C_{q_1}^T \mbox{, \ \  if } k = 2 \\
     & E[\widetilde{\y}(t)\z^T_{w}(t)]=C_{q_k}M_{v}(p_{q_2,q_1}M_{q_2,q_1}P_{q_1}+B_{q_1,q_2}Q_{q_2,q_1}D_{q_1})C_{q_1}^T 
     p_{v}
   \end{split}
   \end{equation}
   In particular,
   $\{\widetilde{\y}(t),\bu_{\sigma}(t)\mid t \in \mathbb{Z}\}$
   satisfies Assumption \ref{gen:filt:ass1:cond0}.
  \end{Lemma}
  \begin{proof}[Proof of Lemma \ref{real:necc_lemma0}]
   Assumption \ref{Assumption2} implies that $\x(t)$ is zero
   mean and that $P_{q}=E[\x(t)\x^T(t)\chi(\btheta(t)=q)]$
   does not depend on $t$.  Notice that
   $\widetilde{\y}(t)=C_{\btheta(t)}\x(t)+D_{\btheta(t)}\v(t)$.
   By Assumption \ref{Assumption4},
   $E[C_{\btheta(t)}\x(t) \mid \mathcal{D}_t]=C_{\btheta(t)}E[\x(t)\mid \mathcal{D}_t]=0$.
   By Assumption \ref{Assumption0},
   $E[D_{\btheta(t)}\v(t) \mid \mathcal{D}_t]=D_{\btheta(t)}E[\v(t)\mid \mathcal{D}_t]=0$.
   Hence, $E[\widetilde{\y}(t)]=E[C_{\btheta(t)}\x(t)]+E[D_{\btheta(t)}\v(t)]=0$.
   Using the state-update equations of $H$,
   it is easy to see that
   the entries of $\widetilde{\y}(t)\z^T_{w}=\y(t)\z^T_{w}(t)$ are linear combinations of
   entries of expressions of the form
   \[
    \begin{split}
     & Z_1:=\x(t-k)\x^T(t-k)\chi(\btheta(t-k)=q_1\cdots \btheta(t)=q_k)] \\
    & Z_{2,l}:=\x(t-k)\v^T(t-l)\chi(\btheta(t-k)=q_1\cdots \btheta(t)=q_k)], l=0,1,\ldots, k, \\
   & Z_{3,l}=\v(t)\v^T(t-l)\chi(\btheta(t-k)=q_1\cdots \btheta(t)=q_k)] l=0,1,\ldots, k \\
  & Z_{4}=E[\v(t-1)\v(t-k)\chi(\btheta(t-k)=q_1\cdots \btheta(t)=q_k)]
  \end{split}
   \]
   By Assumption \ref{Assumption0} that $\v(t)$, $\v(t-l)$ and
   $\x(t-k)$, $\v(t-l)$ are conditionally uncorrelated, we
   get by first conditioning on $\mathcal{D}_{t-k}$ that
   \[
    \begin{split}
     & E[Z_{2,l}\mid \mathcal{D}_{t-k}]=E[\x(t-k)\v(t-l)^T\mid \mathcal{D}_{t-k}]\chi(\btheta(t-k)=q_1)p_{q_1,q_2}\cdots p_{q_{k-1},q_k}=0 \\
   & E[Z_{3,l}\mid \mathcal{D}_{t-l}]=E[\v(t)\v^T(t-l)\mid \mathcal{D}_{t-l}]\chi(\btheta(t-k)=q_1,\ldots,\btheta(t-l)=q_l)p_{q_l,q_{l+1}}\cdots p_{q_{k-1},q_k}=0 \\
  \end{split}
   \]
   Hence, $E[Z_{2,l}]=E[E[Z_{2,l}\mid \mathcal{D}_{t-k}]]=0$ and
  $E[Z_{3,l}]=E[E[Z_{3,l} \mid \mathcal{D}_{t-l}]]=0$.
  By writing out the exact expression for $\y(t)\z_{w}(t)$ and
  taking into account the remarks above and the fact that
  \[ 
     \begin{split}
      & E[Z_1]=E[E[Z_1\mid \mathcal{D}_{t-k}]]=
            p_{q_k,q_{k-1}}\cdots p_{q_1,q_2}E[\x(t-k)\x(t-k)\chi(\btheta(t-k)=q_1)], \\
      & E[Z_4]=E[E[Z_4\mid \mathcal{D}_{t-k+1}]]=
        p_{q_k,q_{k-1}}\cdots p_{q_3,q_2}E[\v(t-k)\v(t-k)\chi(\btheta(t+1)=q_2,\btheta(t)=q_1)]
     \end{split}
   \]
  we obtain that \eqref{real:necc_lemma0:eq1}.
  \end{proof}


%The following definition and lemma explains the relationship between
%family of formal power series $\Psi_{\y}$ and
%the matrices of a GJMLS realization.



%%  \begin{Lemma}[Necessary Conditions]
%%  \label{real:necc_lemma}
%%   If $H$ is a realization of $\widetilde{\y}$, then
%%   $R_{H}$ is a representation of $\Psi_{\widetilde{\y}}$. In particular, if $\widetilde{\y}$ has a GJLS realization, then
%%   $\Psi_{\widetilde{\y}}$ is rational.
%%  \end{Lemma}
%%  \begin{proof}[Proof of Lemma \ref{real:necc_lemma}]
%%   Consider first any
%%   word $v=(q_2,q_3)\cdots (q_{k-1},q_k) \in L$,
%%   $q_1 \ldots q_k \in Q$, $k >0$. It is easy to see
%%   that  all the entries of
%%   $A_{w}$ are zero, except the ones in the sub-matrix
%%   formed by the intesections of the
%%   columns indexed by 
%%    $j \in [n_1+\cdots +n_{q_2-1}+1,n_1+\cdots + n_{q_2}]$ and 
%%   rows indexed by 
%%   $i \in [n_1+\cdots+n_{q_k-1}+1, n_1+\cdots+n_{q_k}]$.
%%   The latter submatrix equals 
%%   %\begin{equation}
%%   %\label{real:necc_lemma:eq1}
%%   \(  p_{v}M_{v}  \).
%%    %p_{q_k,q_{k-1}}\cdots p_{q_3,q_2}M_{q_k,q_{k-1}}\cdots M_{q_3,q_2}
%%   %\end{equation}
%%   From this and the definition of $B_{i, (q_1,q_2)}$, $i=1,\ldots,p$ and $C$ it follows
%%   %that for $w=(q_2,q_3)\cdots (q_{k-1},q_k) \in L$, 
%%   \begin{equation}
%%   \label{real:necc_lemma:eq2}
%%      \begin{split}
%%        & C\begin{bmatrix}
%%               B_{1,(q_1,q_2)} & \ldots & B_{p,(q_1,q_2)}
%%        \end{bmatrix} =CG_{q_1,q_2} \\
%%        & CA_{v}\begin{bmatrix} 
%%               B_{1,(q_1,q_2)} & \ldots & B_{p,(q_1,q_2)}  
%%        \end{bmatrix} = \\
%%       & p_{v}M_{v}G_{q_1,q_2}
%%    \end{split}
%%   \end{equation}
%%   Combining \eqref{real:necc_lemma:eq2} with Lemma
%%   \ref{real:necc_lemma0} and the definition of $G_{q_1,q_2}$
%%   implies that for all $i=1,\ldots,p$, $q_1 \in Q$,
%%   \[ S_{i,(q_1,q_2)}(v)=CA_{v}B_{i,(q_1,q_2)} \]
%%   Moreover, the definition of of $B_{i,(r,s)}$, $i=1,\ldots,p$,
%%   $s \ne q_2$ implies that the rows of $B_{i,(r,s)}$ indexed
%%   by $i \in [n_1+\cdots+n_{q_2-1}+1,n_1+\cdots + n_{q_2}]$ are
%%   zero, and hence $A_{v}B_{i,(r,s)}=0$ for all $i=1,\ldots,p$
%%   and $q_2 \ne s \in Q$. Hence for all pairs $(r,s)$ such that
%%   $s \ne q_2$,
%%  \[ 0=S_{i,(r,s)}(v)=CA_{v}B_{i,(r,s)}=0. \]
%%   Note that $S_{i,(r,s)}(v)$ is the $i$th column of
%%   $\Lambda_{(r,s)w}$ and the latter equals zero since
%%   for $s \ne q_2$, $(r,s)v \notin L$.
%%   
%%   Finally, notice that for any $v \notin L$, $A_{v}=0$. 
%%   Combining all these observations we conclude that
%%   \[ \forall v \in \Sigma^{*}: S_{i,(r,s)}(v)=CA_{v}B_{i,(r,s)} \]
%%   for all $i=1,\ldots,p$, $(r,s) \in Q \times Q$, i.e.
%%   $R_H$ is indeed a representation of $\Psi_{\widetilde{\y}}$.
%%  \end{proof}


The following result characterizes the relationship between Assumptions \ref{Assumption0}--\ref{Assumption2} in Section \ref{sect:GJMLS} about GJMLSs, and Assumptions \ref{real:suff:ass1.1}--\ref{real:suff:ass1.3}.
%
 \begin{Lemma}
 \label{real:suff:lemma1}
If $\widetilde{\y}$ has a realization by a GJMLS for which Assumptions \ref{Assumption0}--\ref{Assumption2} hold, then Assumptions \ref{real:suff:ass1.1}--\ref{real:suff:ass1.3} hold as well.
 \end{Lemma}
 \begin{proof}[Proof of Lemma \ref{real:suff:lemma1}]
  Let $H$ be the GJMLS which is a realization of 
  $\widetilde{\y}$. 

  First we show that $\widetilde{\y}(t)$ satisfies
  Assumption \ref{real:suff:ass1.1}.
  Then by Assumption \ref{Assumption0},
  Part \ref{Assumption0:part2}, $\{\x(t-l),\v(t-l) \mid l \ge 0\}$
  are conditionaly independent of $\{\btheta(t+k) \mid k >0\}$
  with respect to $\mathcal{D}_t=\{\btheta(t-l) \mid l \ge 0\}$.
  But $\widetilde{\y}(t-l)=C_{\btheta(t-l)}\x(t-l)+D_{\btheta(t-l)}\v(t-l)$,
  from which conditional independence of $\{\y(t-l)\}$ and
  $\{\btheta(t+k)\}$ w.r.t. $\mathcal{D}_t$ follows.
  Indeed, let $A$ be any event in the $\sigma$-algebra generated
  by $\{\btheta(t+k) \mid k >0\}$. Then, by exploiting the
  fact that $\chi(\btheta(t-l)=q)$ is $\mathcal{D}_t$ measurable
  and hence for any random variable $X$, $E[X\chi(\btheta(t-l)=q)\mid \mathcal{D}_t]=\chi(\btheta(t-l)=q)E[X\mid \mathcal{D}_t]$, we obtain
  \[
    \begin{split}
     & E[\widetilde{\y}(t-l)\chi(A)\mid \mathcal{D}_t]=
     \sum_{q \in Q} (C_qE[\x(t-l)\chi(A)\mid \mathcal{D}_t]+D_q
      E[\v(t-l)\chi(A)\mid \mathcal{D}_t])\chi(\btheta(t-l)=q)= \\
    & \sum_{q \in Q} (C_qE[\x(t-l)\mid \mathcal{D}_t]+D_{q}E[\v(t-l) \mid \mathcal{D}_t])\chi(\btheta(t-l)=q)E[\chi(A)\mid \mathcal{D}_t] = \\
    & E[\widetilde{\y}(t-l) \mid \mathcal{D}_t]E[\chi(A)\mid \mathcal{D}_t]
  \end{split}
   \]
  In the second step, we used  by Assumption \ref{Assumption0},
  Part \ref{Assumption0:part2}.

  Next we show that $\widetilde{\y}(t)$ satisfies
  Assumption \ref{real:suff:ass1.2}.
  To this end recall the definition of the
  representation $R_H$ associated with the GJLS $H$.
  From Lemma \ref{real:necc_lemma} it follows that
  $R_H=(\mathbb{R}^{n},\{A_{\sigma}\}_{\sigma \in \Sigma},C,B)$  is a representation of $\Psi_{\widetilde{\y}}$.
  %that is,
  %$CA_{w}B_{i,\sigma}=S_{(i,\sigma)}(w)$ for all
  %$w \in \Sigma^{*}$, $\sigma \in \Sigma$, $i=1,\ldots,p$.
  Define the matrix $\widetilde{A}_{(q_1,q_2)}=\frac{1}{\sqrt{p_{q_1,q_2}}} A_{q_1,q_2}$. A straightforward calculation
  reveals that
  \[ \widetilde{M}=\sum_{\sigma \in \Sigma} \widetilde{A}^T_{\sigma} \otimes  \widetilde{A}_{\sigma}^T, \]
  where $\widetilde{M}$ is the matrix from
  Assumption \ref{Assumption1.5}. From Assumption
  \ref{Assumption1.5} it then follows that 
  the representation $\hat{R}=(\mathbb{R}^{n},\{\widetilde{A}_{\sigma}\}_{\sigma \in \Sigma}, C,B)$ is stable.
  For each $i=1,\ldots,p$, $\sigma \in \Sigma$, 
  define the power series 
  $\widetilde{S}_{(i,\sigma)}(w)=C\widetilde{A}B_{(i,\sigma)}$, $w \in \Sigma^{*}$.
  From Theorem \ref{hscc_pow_stab:theo2} it then follows that
  $\widetilde{S}_{(i,\sigma)}$ is square summable.
  From the definition of $\widetilde{A}_{\sigma}$,
  $\sigma \in \Sigma$
  it follows that
  \[ ||\widetilde{S}_{(i,\sigma)}(w)||_{2}^{2} = ||C\widetilde{A}_{w}B_{(i,\sigma)}||_{2}^{2} \ge 
     \frac{1}{K} ||CA_{w}B_{(i,\sigma)}||_{2}^{2}=
     \frac{1}{K} ||S_{(i,\sigma)}(w)||_{2}^{2},
  \]
  where $K=\max\{p_{q,r} \mid q, r\in Q\} > 0$.
  Hence square summability of $\widetilde{S}_{(i,\sigma)}$
  implies square summability of $S_{(i,\sigma)}$, for
  all $i=1,\ldots,p$, $\sigma \in\Sigma$. Hence,
  $\Psi_{\widetilde{\y}}$ is indeed square summable.


  Finally, Assumption \ref{real:suff:ass1.3} is
  identical to  Assumption \ref{Assumption1}.
 \end{proof}

In order to use the results of Section \ref{gen:filt} to derive a realization construction for GJMLSs, we will also need the following assumptions.

%%\begin{Assumption}[Positive definiteness of finite covariance]
%%\label{real:ass1.4} For each pair of admissible words $w,v \in L$, let
%%$T_{v,w}=E[\z_{v}(t)\z_{w}^{T}(t)]$. We assume that the finite matrix 
%%$T^N=(T_{w,v})_{w,v \in L,|w|,|v|\le N}$ formed from admissible words of length at most $N>0$ is strictly positive definite, \ie it satisfies Assumption \ref{gen:filt:ass1:cond3} in Section \ref{gen:filt}.
%%\end{Assumption}
%
 
These assumptions are related to Assumptions \ref{gen:filt:ass1:cond1}--\ref{gen:filt:ass1:cond6} of Section \ref{gen:filt} by the following lemma.
 
\begin{Lemma}
\label{real:suff:lemma2}
If $\widetilde{\y}$ and $\btheta$ satisfy 
Assumption \ref{real:suff:ass1.1}--\ref{real:suff:ass1.5},
then it satisfies Assumptions \ref{gen:filt:ass1:cond1}--\ref{gen:filt:ass1:cond6}.
In particular, Assumption \ref{gen:filt:ass1:cond5} is satisfied with $p_\sigma$ defined as the transition probability of the Markov process $\btheta$, that is, for $\sigma = (q_1,q_2)$, we let $p_{(q_{1},q_{2})}=p_{q_{1},q_{2}}$.
 \end{Lemma}
\begin{proof}[Proof of Lemma \ref{real:suff:lemma2}]
\end{proof}
 
Now we are ready to formulate the main theorem of this section.
%
\begin{Theorem}[Existence of a GJMLS Realization]  
 \label{real:suff:theo1}
  Assume that $\widetilde{\y}$ and $\btheta$ satisfies Assumptions 
  \ref{real:suff:ass1.1}--\ref{real:suff:ass1.5}. Then $\widetilde{\y}$ has a realization by a 
  GJLS system with discrete state $\btheta$ if and only if $\Psi_{\widetilde{\y}}$ 
  is rational.  Furthermore, if $R=(\mathbb{R}^{n}, \{ A_{\sigma} \}_{\sigma \in \Sigma}, \{B_{(i,\sigma)}\}_{i \in I, \sigma \in \Sigma},C)$
  is a minimal representation of $\Psi_{\widetilde{\y}}$,
  then we can define a GJLS $H_{R}$ which is a realization
  of $\widetilde{\y}$ as
%
  \begin{equation}
  H_{R}: \left \{
  \begin{split}
   \hat{\x}(t+1)&=M_{\btheta(t+1),\btheta(t)}\hat{\x}(t)+
                 K_{\btheta(t+1),\btheta(t)}\e(t)  \\
   \widetilde{\y}&=C_{\btheta(t)}\hat{\x}(t) + \e(t), 		 \end{split}		 
  \right.
  \end{equation}
%
  where 
%
\begin{enumerate}
\item 
 \textit{Continuous state-spaces. }
  For each $q \in Q$ define 
  $\mathcal{X}_{q} \subseteq  \mathbb{R}^{n}$ 
  as the subspace spanned
  by all the elements
  of the form $A_{(q_{1},q)}A_{w}B_{(i,\sigma)}$ and
  $B_{(i,(q_{1},q))}$ for all
  $q_{1} \in Q$, $w \in \Sigma^{+}$, $\sigma \in \Sigma$,
  $i=1,\ldots, p$. Then identify the elements of $\mathcal{X}_{q}$
  with the elements of $\mathbb{R}^{n_q}$, where $n_{q}=\dim \mathcal{X}_{q}$.
  %
\item  
\textit{State process.} 
The continuous state process $\hat{\x}(t)$ of the GJMLS is  obtained from the continuous state $\x(t)$ of the generelizad bilinear system \ref{gen:filt:eq2} by viewing it as an element of $\mathcal{X}_{\btheta(t)}$ and identifying it with the corresponding vector in $\mathbb{R}^{n_{q}}$ for $q=\btheta(t)$.
%
\item  
\textit{System matrices.} 
For each $q_1,q_2 \in Q$ the matrix $M_{q_{1},q_{2}} \in \mathbb{R}^{n_{q_{2}} \times n_{q_1}}$ is the matrix associated with the linear map 
%
\begin{equation}
\mathcal{X}_{q_{1}} \ni x \mapsto \frac{1}{p_{q_1,q_2}}
     A_{q_{1},q_{2}}x \in  \mathcal{X}_{q_{2}} .
\end{equation}
%
For each $q \in Q$ the matrix $C_{q} \in \mathbb{R}^{p \times n_{q}}$ is the matrix associated with the linear map $\mathcal{X}_{q} \ni x \mapsto Cx \in \mathbb{R}^{p}$, \ie 
$C_{q}$ is the restriction of $C$ to $\mathcal{X}_{q}$.
%
\item 
\textit{Innovation process. } 
The process $\e(t)$ is the innovation process, \ie 
  \begin{equation}
   \begin{split}
     \e(t) =\widetilde{\y}(t)-E_{l}[\widetilde{\y}(t) \mid &
         \{ \widetilde{\y}(t-k)\chi(\btheta(t-k)=q_{1})\cdots \\
	    & \chi(\btheta(t)=q_{k}) \mid 
	    q_{1},\ldots, q_{k} \in Q, k \ge 0\}]. 
   \end{split}	    
  \end{equation}
  That is, $\e(t)$ is the difference between
  $\widetilde{\y}(t)$ and its projection onto the subspace
  formed by the predictor variables 
  $\widetilde{\y}(t-k)\chi(\btheta(t-k)=q_{1}) \cdots \chi(\btheta(t)=q_{k})$, 
  $k \ge 0$, $q_{1},\ldots, q_{k} \in Q$.
%
\item 
\textit{Noise gain. } 
Let the matrices $B_{q_1,q_2}$ be defined as follows.
Each vector $B_{(i,(q_1,q_2))}$ is an element of $\mathcal{X}_{q_2}$ 
and hence can be identified uniquely with a vector in $\mathbb{R}^{n_{q_2}}$.
%
With this identification let  
%$B_{q_{1},q_{2}}$ be the $n_{q_{2}} \times p$ matrix 
%
\begin{equation}  
 B_{q_1,q_2}=
 \begin{bmatrix} 
 B_{(1,(q_1,q_2))}, & B_{(2,(q_1,q_2))}, & \cdots , & B_{(p,(q_1,q_2))}
  \end{bmatrix}  \in \Re^{n_{q_2}\times p}.
 \end{equation}
Let $T_{(q_1,q_{2}),(q_1,q_2)}$ be the self covariance of $\widetilde{\y}(t)\chi(\btheta(t)=q_1,\btheta(t+1)=q_2)$, \ie
%
\begin{equation} 
T_{(q_1,q_2),(q_1,q_2)} =
E[\widetilde{\y}(t)\widetilde{\y}^{T}(t)\chi(\btheta(t)=q_1,\btheta(t+1)=q_2)] \in\Re^{p\times p}.
\end{equation}
%
Moreover, let $P_{q_1,q_{2}}$ be the self covariance of $\hat{\x}(t)\chi(\btheta(t)=q_1,\btheta(t+1)=q_2)$, \ie
\begin{equation}
P_{q_{1},q_{2}}=E[\hat{\x}(t)\hat{\x}^{T}(t)\chi(\btheta(t)=q_1,\btheta(t+1)=q_2)]
     \in \mathbb{R}^{n_{q_1} \times n_{q_1}}.
\end{equation}
%
The matrix $K_{q_{1},q_{2}} \in \mathbb{R}^{n_{q_{2}} \times p}$ is defined as 
  \begin{equation}
  \begin{split}
  K_{q_{1},q_{2}}&=(B_{q_{1},q_{2}} - \frac{1}{p_{q_{1},q_2}}
      M_{q_{1},q_{2}}P_{q_1,q_2}C_{q_1}^{T}) 
       (T_{(q_1,q_2),(q_1,q_2)}- p_{q_1,q_2} C_{q_1}P_{q_1,q_2}C_{q_1}^{T})^{-1}
  \end{split}    
  \end{equation}
  %
\end{enumerate} 

%Moreover, if we denote by $P_{q}$ the covariance
%%$E[\x(t)\x^{T}(t)\chi(\btheta(t)=q)]$, then 
%%\[ P_{q}=\sum_{q_{1} \in  Q} p_{q,q_1}M_{q,q_1}P_{q_{1}}M_{q,q_1}^{T}+K_{q,q_{1}}Q_{q,q_1}K_{q,q_1}^{T} \]
%%where $Q_{q,q_1}=E[\e(t)\e(t)^{T}\chi(\btheta(t)=q_1,\btheta(t+1)=q)]$.
%%\end{enumerate}

The system $H_{R}$ is a well-defined GJMLS and
it satisfies Assumptions \ref{Assumption0}--\ref{Assumption2}.
%%The realization $H_{R}$ is a minimal GJMLS realization
%%of $\widetilde{\y}$.
\end{Theorem}  
\begin{proof}[Sketch]
 First, we prove necessity, that is, we will
 show that if $\widetilde{\y}$ has a GJLS realization,
 then $\Psi_{\widetilde{\y}}$ is rational.
The proof that $H_{R}$ is a GJLS realization of $\widetilde{\y}$ follows from Theorem \ref{gen:filt:theo3}.  \end{proof}
 %%Follows from Theorem \ref{gen:filt:theo3}.
  %To this end,  
   %%minimal representation of $\Psi_{\widetilde{y}}$.
%%   Define the representation  $\hat{R}$
%%   as follows.
%%   \begin{Construction}
%%   \label{hat:const}
%%   Let $\hat{R}$ be a representationf of the form
%%   \begin{equation}
%%   \label{real:suff:hat:eq}
%%   \hat{R}=(\mathcal{X}, \{ \hat{M}_{\sigma} \}_{\sigma \in \Sigma}, \hat{B}, \hat{C}) 
%%   \end{equation}
%%   where
%%   \begin{enumerate}
%%   \item \textbf{The state-space $\mathcal{X}$} \\
%%     For each $q \in Q$ define the subspace $\mathcal{X}_{q}$
%%     of $\mathbb{R}^{n}$ as the linear space spanned
%%     by vectors of the form $M_{q}M_{w}B_{(i,q)}$ and $B_{(i,q)}$
%%     for all $i=1,\ldots, p$ and $w \in Q^{*}$, i.e.
%%     \begin{equation}
%%     \label{cont:state:space}
%%      \mathcal{X}_{q}=\SPAN\{ M_{q}M_{w}B_{(i,q)}, B_{(i,q)}
%%         \mid w \in Q^{*}, i=1,\ldots, p \}
%%     \end{equation}
%%     Assume that $n_{q}=\dim \mathcal{X}_{q}$ and let 
%%     $N=\sum_{q \in Q} n_{q}$. With this notation, let
%%     $\mathcal{X}=\mathbb{R}^{N}$. Note that 
%%     $\mathcal{X}$ is isomorphic to, and hence can be identified
%%     with, the direct sum of the vector spaces $\mathcal{X}_{q}$,
%%     $q \in Q$, i.e. $\mathcal{X} \cong \bigoplus_{q \in Q} \mathcal{X}_{q}$.
%%     
%%   \item \textbf{ The matrices $\hat{M}_{\sigma}$, $\sigma \in \Sigma$} \\
%%       For each $(q_{1},q_{2}) \in \Sigma$, define the
%%       matrix $\hat{M}_{(q_{1},q_{2})} \in \mathbb{R}^{N \times N}$
%%       as follows. Let $\hat{M}_{(q_{1},q_{2})}$ be the
%%       matrix representation of the linear map
%%       \( \hat{M}_{(q_{1},q_{2})}: 
%%            \bigoplus_{q \in Q} \mathcal{X}_{q} \rightarrow
%%	    \bigoplus_{q \in Q} \mathcal{X}_{q}
%%        \)	    
%%      define as $\hat{M}_{(q_{1},q_{2})}x=M_{q_{2}}x \in \mathcal{X}_{q_{2}}$ for
 %%The above lemma implies that we can apply Theorem \ref{gen:filt:theo3} to solve the realization problem for GMLJs with fully 
 %%observed discrete state.
 %%\begin{Lemma}
 %%\label{real:suff:lemma3}
 %% If $R$ is a stable representation, then $\hat{R}$ is a 
 %% stable representation as well. 
 %%\end{Lemma}
 %%\begin{proof}
   %%Follows easily from Lemma \ref{hscc_pow_stab:lemma1}.
 %%\end{proof}
%% \begin{Corollary}
%% \label{real:suff:col1}
%%  Assumption \ref{real:suff:ass1} holds, and $R$ is a 
%%  minimal representation of $\Psi_{\widetilde{\y}}$, then
%%  the representation $\hat{R}$ constructed from is stable.
%% \end{Corollary} 
%% \begin{proof}
%%  Notice that Assumption \ref{real:suff:ass1} implies that
%%  $\Psi_{\widetilde{\y}}$ is square summable, and hence
%%  by Theorem \ref{hscc_pow_stab:theo} $R$ is stable.
%%  The from Lemma \ref{real:suff:lemma3} it follows that $\hat{R}$
%%  is stable.
%% \end{proof}.
%% In fact, it turns out that if $\widetilde{\y}$ is realized
%% by a GMJLS and $R$ is a minimal representation of 
%% $\Psi_{\widetilde{\y}}$, then  $\hat{R}$ yields a 
%% minimal GJMLS realization of $\widetilde{\y}$.
%% \begin{Lemma}
%% \label{real:suff:lemma3}
%%  If $R$ is a minimal representation of $\Psi_{\widetilde{\y}}$,
%%  then for any GJLS system realization $\Sigma$ of $\widetilde{\y}$,
%%  $\dim \Sigma \ge \dim \hat{R}$.
%% \end{Lemma}
%%  We will use Theorem \ref{gen:filt:theo3} to construct
%%  a GJMLS realization of $\widetilde{\y}$.
%%Notice that by construction of
%%$\hat{R}$, for each $w(q_{1},q_{2}) \in L$, 
%%$\widetilde{\Lambda}_{w(q_{1},q_{2}))} \in \mathcal{X}_{q_{2}}$
%%and hence it can be shown that
%%$\alpha_{w(q_{1},q_{2})} \in \mathcal{X}_{q_{2}}$. Moreover,
%%for any $t$, $z_{w(q_{1},q_{2})}(t)=0$ if $q_{2} \ne \btheta(t)$,
%%hence $\x(t) \in \mathcal{X}_{q_{2}}$ if $q_{2}=\btheta(t)$.
%%Similarly, we get that $K_{q_{1},q_{2}} \in \mathcal{X}_{q_2}$.
%%Noticing that the restriction of $A_{(q_{2},q_{1})}$
%%maps $\mathcal{X}_{q_2}$ to $\mathcal{X}_{q_1}$ and viewing
%%the state at time $t$ as an element of $\mathcal{X}_{\btheta(t)}$
%%instead of $\mathcal{X}$ we obtain the state equation of
%%$H$.
%%Finally, we notice that $\dim \Sigma=\dim \hat{R}$, which 
%%implies 
%%The proof of minimality of $H_{R}$ is a bit more
%%elaborate and we will skip it for lack of space.
%%\end{proof}
%%The theorem above bears a great deal of resemblence to the
%%classical stochastic linear realization theory. It also
%%yields a characterization of minimality
%%in terms of reachability and observability. 

\subsection{Minimality of Realization by a GJMLS with Fully Observed Discrete States}
\label{real:min}


Recall the notion of \emph{minimality} of a realization by a linear stochastic system \cite{Caines1}. In particular, recall that a realization by a linear system is minimal if and only if it is reachable and observable. In this subsection, we will formulate similar concepts for GJMLS with fully observed discrete. We first define the notions of reachability and observability for a GJMLS. We then show that a realization by a GJMLS is minimal if and only if it is reachable and observable. 

In order to formulate the conditions more precisely, we will need to introduce some notation. In particular, we need to define reachability and observability matrices for GJMLS.
% 
To that end, let $H$ be a given GJLS of the form \eqref{stoch_jump_lin:geq1}
that satisfies Assumptions \ref{Assumption0}--\ref{Assumption2}.
%
Let $N$ be the dimension of $H$, i.e. $N=\dim H$, and for all $(q_1,q_2)\in Q\times Q = \Sigma$
let 
\begin{align}
G_{q_1,q_2}=E[\x(t)\y^{T}(t-1)\chi(\btheta(t)=q_2,\btheta(t-1)=q_1)] \in \Re^{q_2 \times p}.
\end{align}
%
Recall the definition of $L \subset Q \times Q=\Sigma$ from (\ref{real:suff:admiss1}).
% 
%
For each $q\in Q$, $L^{q}(N)$ be the set of all words in $L$ of length at most $N$ that end in some pair whose second component is $q$, \ie $L^{q}(N)$ is the set of all words in $w \in L$ such that $|w| \le N$ and $w=v(q_1,q)$ for some $q_1 \in Q$ and $v \in L$.

%%\begin{equation}
%%L_q^N = \{ w \in L \mid |w| \le N 
%%\text{   and   } 
%%\exists q_1 \in Q, v \in L, \qquad  w=v(q_1,q) \}
%%\end{equation}
%For any admissible word $w=(q_1,q_2)v \in L$, let
%$R_{w}=M_{v}P_{q_1}$, where $P_{q_1}\in\Re^{q_1\times q_1}$ is the matrix defined
%in Assumption \ref{Assumption2}. Then 
%for any $w \in L^{N}_q$ the matrix $R_{w}$ is an
%$n_{q} \times p$ matrix.

\begin{Definition}[Reachability of a GJMLS]
For each discrete state $q \in Q$, define the matrix
\begin{equation}
%R_{H,q}=[ R_{w} \mid w \in L^{N}_{q} ]  \in \Re^{n_q \times |L^{N}_{q}|p}.
R_{H,q}=[ M_{v}G_{q_1,q_2} \mid q_1 \in Q , q_2 \in Q, (q_1,q_2)v \in L^q(N) ]  \in \Re^{n_q \times |L^q(N)|p}.
\end{equation}
% 
We will say that the GJMLS $H$ is \emph{reachable}, if for each discrete
state $q \in Q$, $\Rank (R_{H,q}) = n_{q}$. 
\end{Definition}
%
Notice that the matrix $R_{H,q}$ is analogous to the controllability matrix for linear systems. 

For each $q\in Q$, let $L_{q}(N)$ be the set of all words in $L$ of length at most $N$ that begin in some pair whose first component is $q$, \ie $L_{q}(N)$ is the set of all words in $w \in L$ such that $|w| \le N$ and $w=(q,q_2)v$ for some $q_2 \in Q$ and $v \in L$.
%
\begin{Definition}[Observability of a GJMLS]
For each discrete state $q \in Q$, define the matrix
\begin{align}
%O_{H,q}= \bigcap_{q_{k-1} \in Q, q_k \in Q, v(q_{k-1}, q_k) \in L_q(N)]^T  } \ker (C_{q_k} M_v) \\
O_{H,q}=[ (C_{q_k} M_v )^T  \mid q_{k-1} \in Q, q_k \in Q, v(q_{k-1}, q_k) \in L_q(N)]^T  \in \Re^{| L_q(N) |p \times n_q}.
\end{align}

%subspace
%$O_{H,q}$ of $\mathcal{X}_{q}$ as the intersection of
%all the kernels $\ker C_{q_3}M_{w}M_{q_1,q}$, for all
%$(q,q_1)w(q_2,q_3) \in L^{N}$,
%where $L^{N}$ denotes the set of all
%words of $L$ of length at most $N$, i.e.
%%
%\begin{equation}
%O_{H,q}=\bigcap_{(q,q_1)w(q_2,q_3) 
%           \in L^{N},q_1,q_2,q_3 \in Q}
%            \ker C_{q_3}M_{q_3,q_2}M_{w}M_{q_1,q} .
%\end{equation}
%
We will say that a GJMLS $H$ is \emph{observable}, if for each discrete state $q \in Q$, 
$\Rank (O_{H,q}) = n_q$.
%$O_{H,q}=\{0\}$, i.e. the space $O_{H,q}$ is trivial.
\end{Definition}
%
Notice that the matrix $O_{H,q}$ plays a role similar to the observability matrix for linear systems. 
%Notice that the space $O_{H,q}$ plays a role similar to the kernel of the observability matrix for linear systems. 

Recall from (\ref{real:gjmls_repr}) the definition of the representation $R_{H}$ associated with a GJLS $H$ and recall the definition of reachability of a representation along with the definition of the space $O_{R_{H}}$ defined in (\ref{sect:pow:form1.1}). Observability and reachability of a GJMLS $H$ can be characterized in terms of the observability and reachability of the corresponding representation $R_{H}$ as follows. 

\begin{Lemma}
\label{real:lemma:reachobs}
The GJMLS
$H$ is reachable if and only if $R_{H}$ is reachable, and
$H$ is observable if and only if for each $q \in Q$,
$O_{R_{H}} \cap \mathcal{X}_{q}=\{0\}$.
\end{Lemma}
The lemma above implies that observability and reachability of a GJMLS can 
be checked by a numerical algorithm.

We are now ready to state the theorem on minimality of a GJMLS realization.
%
\begin{Theorem}[Minimality of a realization by a GJMLS]
\label{real:theo:min}
Let $\widetilde{\y}$ be an output process satisfying Assumptions \ref{real:suff:ass1.1}--\ref{real:suff:ass1.5}. Let the GJMLS $H$ be a realization of $\tilde\y$ of the form 
\eqref{stoch_jump_lin:geq1}. Then, the GJMLS $H$ is a minimal realization of $\widetilde{\y}$ if and only if it is reachable and observable. 
%
In addition, if $\hat{H}$ is another GJMLS realization of $\widetilde{\y}$ given by
 \begin{eqnarray*}
 \hat{\x}(t+1)&=&\hat{M}_{\btheta(t),\btheta(t+1)}\hat{\x}(t)+
         \hat{B}_{\btheta(t),\btheta(t+1)}\hat{\v}(t) \\
 \hat{\y}(t)&=&\hat{C}_{\btheta(t)}\hat{\x}(t) + \hat{D}_{\btheta(t)}\hat{\v}(t), 	 
 \end{eqnarray*}
 where the dimension of the continuous state-space of $\hat{H}$
 corresponding to the discrete state $q$ is
 $\hat{n}_{q}$, then the GJMLS $\hat{H}$ is minimal if and only if 
 $n_{q}=\hat{n}_{q}$ for all $q \in Q$. 
 %
 Furthermore, there exists a collection of nonsingular matrices,  
 $T_{q}\in\Re^{n_q\times n_q}$, $q \in Q$, such that for all $q_1,q_2 \in Q$
%
\begin{equation}
\label{isomorph}
T_{q_2}M_{q_1,q_2}T_{q_1}^{-1}=\hat{M}_{q_1,q_2}, \quad
C_{q_1}T^{-1}_{q_1}=\hat{C}_{q_1}, \quad 
T_{q_2}G_{q_1,q_2}=\hat{G}_{q_1,q_2},
\end{equation}
 %
where
%% $G_{q_2,q_1}=(p_{q_1,q_2}M_{q_1,q_2}P_{q_2}+B_{q_1,q_2}W_{q_1,q_2}D_{q_2})C_{q}^{T}$  and 
 %%$\hat{G}_{q_2,q_1}=(p_{q_1,q_2}M_{q_1,q_2}\hat{P}_{q_2}+\hat{B}_{q_1,q_2}\hat{W}_{q_1,q_2}\hat{D}_{q_1,q_2})\hat{C}_{q}^{T}$, and $P_{q}=E[\x(t)\x(t)\chi(\btheta(t)=q)]$, 
 %%$\hat{P}_{q}=E[\hat{\x}(t)\hat{\x}(t)\chi(\btheta(t)=q)]$ for all $q \in Q$.
\begin{align} 
\begin{split}
G_{q_1,q_2} &= E[\x(t)\y^{T}(t-1)\chi(\btheta(t)=q_2,\btheta(t-1)=q_1)],  \quad\text{and}\\
\hat{G}_{q_1,q_2} &=E[\hat{\x}(t)\hat{\y}^{T}(t-1)\chi(\btheta(t)=q_2,\btheta(t-1)=q_1)].
\end{split}
\end{align}
%
That is, $\bar{H}$ and $H$ are algebraically similar in some sense.
\end{Theorem}
%
\begin{proof}[Sketch]
 First, we can show that if $R$ is a minimal
 representation of $\Psi_{\widetilde{\y}}$, then
 the GJLS
 $H_{R}$ defined in Theorem \ref{real:suff:theo1}
 is a minimal realization of $\widetilde{\y}$.
 Moreover, using Lemma \ref{real:lemma:reachobs}
 we can show that $H_{R}$ is reachable and observable.
%%The proof relies on the fact that if $R$ is a minimal
%%representation of $\Psi_{\widetilde{\y}}$, then we can
%%construct a minimal GJLS realization $H_{R}$ of
%%$\widetilde{\y}$ as described in Theorem \ref{real:suff:theo1}.
Assume that 
$\bar{H}$ is a reachable and observable GJLS realization
of $\widetilde{\y}$.
Consider the representation $R_{\bar{H}}$ and 
transform it to a minimal representation $\bar{R}$.
Construct the GJLS $H_{\bar{R}}$. Then we can show 
that $\bar{H}$ and
$H_{\bar{R}}$ are isomorphic and hence $\bar{H}$ is minimal.
The rest of the theorem follows from the properties of
minimal rational representations. We omit the details
due to lack of space.
\end{proof}
%%\begin{Remark}
 %%The proof of Theorem \ref{real:theo:min} resembles the
 %%proof of minimality of the so called hybrid representations
 %%described in \cite{MP:HybPow} and 
 %%\cite{MP:Phd}. 
%% In fact, instead of using rational
%% representations we could use hybrid representations
%% for representing the sequences of covariances.
%% In that case the theorem above follows
%% from the general result on minimality of hybrid representations,
%% see \cite{MP:Phd,MP:HybPow}.
%%\end{Remark}
\begin{Remark}
 Notice that in (\ref{isomorph}) we do not require 
 any relationship between $B_{q_1,q_2}$ and $\hat{K}_{q_1,q_2}$.
 This is consistent with the situation for linear stochastic
 systems.
%% where two minimal realizations can have completely
 %%different $B$ matrices and only the $A$, $C$ and $G$ matrices
 %%are related.
\end{Remark}  
\begin{Remark}[Realization Algorithms]
 It is clear that reachability and observability, and hence 
 minimality, of a GJLS can be checked
 numerically. It is also easy to see that the
 algorithm sketched in Remark \ref{gen:filt:ident}
 can be adapted to obtain the realization $H_{R}$
 described in Theorem \ref{real:suff:theo1}.
\end{Remark}


==> JMLS_real_generalized_main_result.tex <==
\subsection{Informal presentation of the main results}
In this paper we will present the solution of the realization problem for \GBS{s}. More
precisely, we will prove the following.
\begin{Theorem}[Existence and minimality]
 \label{main:theo}
 A process $\y$ is realizable by a \GBS\ if and only if $\y$ satisfies certain technical
 conditions. Minimal \GBS\ realizations of $\y$ are unique
 up to isomorphism, a realization is minimal if and only if it is reachable and observable.
  Moreover, this minimal realization can be chosen to be
 in forward innovation form, i.e. the Kalman-filter of this \GBS\ is the \GBS\ itself.
\end{Theorem}
 Of course, the theorem above is not a theorem in the strict sense of the word, 
 since we did not specify exactly what those `technical conditions' are.  In addition,
 for the theorem to hold, we have to make some mild assumptions on the \GBS{s} involved.
 At this stage, we will not try to define these concepts formally.
 The formal statement of the technical conditions on $\y$ will be presented in
 Assumption \ref{output:assumptions}. The formal definition of the subclass of \GBS{s}
 considered will be presented in Assumption \ref{gbs:def}. Finally, the formal statement
 of the results of Theorem \ref{main:theo} will be presented in Theorem \ref{gen:filt:theo3}--\ref{gen:filt:min_theo}.

 In addition to Theorem \ref{main:theo}, we will also present a realization algorithm which
 computes an approximate realization of $\y$ based on finitely many sampled data points.
 We also show that if the number of the data points goes to infinity, the corresponding
 approximate realizations converge to a true realization of $\y$.

 Instead of formal definitions, below we will try to sketch the main ideas and
 intuitive meaning of Theorem \ref{main:theo}. This will be done by using the analogy
 with linear stochastic realization theory from \cite{Caines1,Katayama:05}.
 We will deal with wide-sense
 stationary linear systems of the form
 \begin{equation*}
 \mathbf{S} \left\{ \begin{split}
   & \x(t+1) = A\x(t)+B\v(t) \\
   & \y(t)   = C\x(t)+D\v(t),
 \end{split}\right.
 where $\v$ is a colored noise, i.e. $\v$ is zero mean, wide-sense stationary,
 $E[\v(l)\v^T(k)]=\delta_{k,l}Q$, where $\delta_{k,l}$ is the Kronecker symbol.
 In order to ensure that $\x(t)$ and $\y(t)$ are wide-sense stationary processes,
 it is commonly assumed that $A$ is stable matrix. In that case, any state trajectory
 of the linear stochastic system $(A,B,C)$ will converge to the stationary state process
 $\x$. In addition, we assume that $\x$ and $\y$ are zero-mean process.
 With the stochastic system $\mathbf{S}$ we can associate a \emph{deterministic linear
 system} $\mathbf{S}_{det}=(A,G,C,\Lambda_0)$, where 
 $G=APC^T+BD^T$, $\Lambda_0=CPC^T+DQD^T$ and $P=E[\x(t)\x^T(t)]$. 

 Consider a wide-sense stationary zero-mean process $\y$. For positive $k,l > 0$, define
 \begin{equation}
 \label{main_theo:eq1}
   \Lambda_k=E[\y(t)\y^T(t-k)] \mbox{ and } T_{k,l}=E[\y(t+k)\y^T(t-l)],
 \end{equation}
 and let $\Lambda_0=E[\y(t)\y^T(t)]$.
%
%
%From wide-sense stationarity of $\y$ it follows that $\Lambda_k$, $k \ge 0$ and 
% $T_{k,l}$, $k,l \ge 0$ are well-defined. Moreover, $T_{k,l}$ satisfies the following
% recursivity property 
% \begin{equation}  
% \label{main_theo:eq2}
%  T_{k+1,l+1}=T_{k,l} \mbox{ and } T_{k+1,1}=\Lambda_k^T 
% \end{equation}
% Another important property of an output process $\y$ arising from a linear system
% is that $\Lambda_k$ is the Markov-parameter ($k$th impulse response) of a 
% \emph{deterministic} linear system $(A,G,C)$, where
% $G=APC^T+BD^T$ and $P=E[\x(t)\x^T(t)]$. In other words,
% \begin{equation}
% \label{main_theo:eq3}
% \Lambda_k=CA^{k-1}G. 
% \end{equation}
 %In fact, conditions \eqref{main_theo:eq2} and \eqref{main_theo:eq1} are 
 %sufficient for existence of a linear system realization of $\y$. More precisely,
 %assume that $\y$ is a stochastic process which satisfies the following conditions.
 Let us make the following assumptions on $\y$.
 \begin{Assumption}
 \label{main:theo:outputs}
 \begin{enumerate}
 \item 
  \label{main:theo:cond1}
  $\y$ is zero mean and it is wide-sense stationary.
 \item
  \label{main:theo:cond2}
 The recursive relationship \( T_{k+1,l+1}=T_{k,l} \mbox{ and } T_{k+1,1}=\Lambda_k^T \)  
 holds for all $k \ge 0$.
 \footnote{
  The attentive reader might have notices that the second condition is a consequence of the first one. However, for our discussion we prefers to state this condition
  separately, since an analogous condition will be required for \GBS{s}.}.
 \item
  \label{main:theo:cond3}
  There exists a minimal stable deterministic linear system 
  $(A,C,G,R)$ with $p$ inputs and $p$ outputs such that
  $\{\Lambda_k\}_{k=0}^{\infty}$ are the Markov-parameters of this system, i.e.
  $R=\Lambda_0$ and $\Lambda_k=CA^{k-1}G$, $k \ge 1$.
 \end{enumerate}
 \end{Assumption}
 For our purposes, we can sum up the main results of linear stochastic realization theory as follows.  
 \begin{Theorem}[\cite{Caines1,Katayama:05}]
  \begin{description}
  \item{Existence of a realization}
    The process $\y$ is realizable by a linear stochastic system if and only if it
    satisfies Assumption \ref{main:theo:cond}.
  \item{Necessity}
    If $\mathbf{S}$ is a stochastic realization of $\y$, then
    $\{\Lambda_k\}_{k=0}^{\infty}$ are the Markov-parameters of the associated
    deterministic system $\mathbf{S}_d$.

  \item{Sufficiency}
   If $\y$ satisfies Assumption \ref{main:theo:cond}, and $(A,G,C,R)$ is a 
   minimal stable linear system whose $k$th Markov-parameter is $\Lambd_k$, then  
   $\y$ has a stochasti realization of the form: 
     
  \item{Minimality}
     A stochastic system $\mathbf{S}$ is a minimal realization of $\y$ if and only
     if the associated deterministic system $\mathfb{S}_{det} is reachable and observable.
     If $\mathbf{S}_1$ and $\mathbf{S}_2$ are two stochastic realizations of $\y$, then
     the deterministic systems associated with them are isomorphic.
  \end{Theorem}
 Moreover, we can choose the stochastic system to be of the form
 \begin{align*}
   \x(t+1) =& A\x(t)+K\e(t) \\
   \y(t)   =& C\x(t)+\e(t),
 \end{align*}
 where $\e(t)=\y(t)-E_l[\y(t) \mid \{ \y(l) \mid l \ge 0\}]$.
 Here $E_l[X\mid Z]$ denotes the orthogonal projection (in the mean-square sense) of
 the random variable $X$ onto the space spanned by elements of $Z$. If all the
 variables are Gaussian (which is often an assumption in the linear case), 
 then $E_l[X \mid Z]$ is simply the conditional expectation of $X$ given the
 variables $Z$. This means that the Kalman-filter for the linear system $(A,C,K)$  
 is the system itself. 

 Moreover, $K$ can be computed from the data
 $(A,C,G, \Lambda_0)$ by solving the algebraic Riccati equation. 
 In turn, $(A,C,G)$ can be obtained from finitely many covariances
 $\Lambda_k$, $k > 0$, using the deterministic realization algorithm by Ho-Kalman.
 The covariances $\Lambda_k$, $k > 0$, can be estimated from data directly.
 In fact, the well-known subspace identification algorithms rely indirectly on
 these facts.

  The discussion above indicates that there is a correspondence 
  between stochastic systems $(A,B,C,D)$ and stable deterministic linear systems
  $(A,C,G,\Lambda_0)$.  This correspondence is onto and preserves dimensionality.
  %Hence, minimality of $(A,B,C,D)$ is equivalent to minimality of the deterministic
  %linear system $(A,C,G,\Lambda_0)$.  
  It then follows that 
  $(A,B,C,D)$ is minimal if and only if the corresponding deterministic
  system $(A,C,G,\Lambda_0)$ is reachable and observable.  Moreover,
  if $(A,B,C,D)$ and $(\hat{A},\hat{B},\hat{C},\hat{D})$ are two minimal
  stochastic realizations of $\y$, then the corresponding deterministic
  linear system $(A,C,G,\Lambda_0)$ and $(\hat{A},\hat{C},\hat{G},\Lambda_0)$
  are isomorphic. Hence, if we define reachability and observability of
  a stochastic system as reachability and observability of the 
  deterministic system $(A,C,G,\Lambda_0)$, then  we can say that
  minimality is equivalent to observability and reachability. If we introduce the
  terminology that two stochastic systems $(A,B,C,D)$ and $(\hat{A},\hat{B},\hat{C},\hat{D})$ are isomorphic if the corresponding deterministic systems
  $(A,B,C,D)$ and $(\hat{A},\hat{B},\hat{C},\hat{D})$ are isomorphic, then
  we can say that minimal stochastic realizations of $\y$ are isomorphic. 

   Note that the correspondence between $(A,B,C,D)$ and $(A,C,G,\Lambda_0)$ is
   \emph{not one-to-one}. Several stochastic systems can yield the same
   deterministic system. In frequency domain, the transfer function
   of $(A,C,G,\Lambda_0)$ corresponds to the power spectrum $\Phi(z)$ of 
   the output process $\y$. The transfer function $H(z)$ of $(A,B,C,D)$ represents a 
   factorization $\Phi(z)=H(z)H(\frac{1}{z})^{T}$ of the power spectrum.
   It is known that such a factorization is not unique. 
   
 
 We will now describe the intuition behind Theorem \ref{main:theo} using 
 the analogy with linear stochastic realization theory.
 The assumption on \GBS{s} is that the system is a stationary
 stochastic system.
 In order to ensure this, we have to assume that the \GBS{s} is stable in a certain sense, and that
 the state process is that state trajectory to which the system converges if started from
 any initial state and perturbed by a colored noise. 
 This is analogous to the standard assumptions on stationary stochastic systems
 discussed above.

 The technical conditions which $\y$ must satisfy involve the following. 
 First, it is assumed
 that $\y$ and the $\bu_{\sigma}$ are jointly (wide-sense) stationary, i.e.
 an extensions of Part \ref{main:theo:cond1} of Assumption \ref{main:theo:outputs}.
 Second, the 
 covariances of the products of past inputs with future outputs exhibit a certain
 recursive property. This is an extension of Part \ref{main:theo:cond2} of
 Assumption \ref{main:theo:outputs}.
 Finally, the covariances of current outputs with products of 
 past outputs and inputs should form a \emph{rational formal power series}, or,
equivalently,
 they should outputs of a deterministic bilinear system. 
 This is a direct extension of Part \ref{main:theo:cond1} of Assumption \ref{main:theo:outputs}.

As in the linear case, the last assumption is the 
one which guarantees the existence of a 
 \GBS{s}. Such a  \GBS\ can, in fact, be obtained from a minimal deterministic bilinear system
 (or, which is equivalent, the rational representation) which generates the covariances.
 In addition, the thus obtained \GBS\ is in forward innovation form. The latter means that
 its noise process is the difference between the actual output and the output predicted
 based on past outputs and inputs. Thus, the state of such systems can be estimated from
 output, or in other words, the system functions as its own Kalman-filter. Hence, such systems
 are interesting for control. 

 Just as in the linear case, we can show that there is a onto correspondence
 between \GBS{s} and deterministic bilinear systems (rational representations)
 generating the covariance sequences. This correspondence preserves minimality.
 Since by \cite{Son:Real,Isidori:TAC73} minimality of deterministic
 bilinear systems (rational representations) is equivalent to observability
 and reachability and equivalent minimal realizations are isomorphic, we can easily
 derive the minimality conditions of Theorem \ref{main:theo}.
 To this end, we just have to choose the definitions of observability,
 reachability and isomorphism of \GBS{s} so that it becomes 
 equivalent to reachability, observability and isomorphism of the
 corresponding deterministic bilinear systems which generates the output covariances.

 Similarly, to the linear case, one can formulate a Kalman-Ho-like realization
 algorithm for bilinear systems (rational representations), see 
 \cite{Son:Real,Isidori:TAC73}. Hence, after estimating the corresponding 
 covariances from the data, we can apply bilinear realization algorithm to 
 obtained covariances to find a deterministic bilinear system generating them.
 From this deterministic bilinear system we can then compute a \GBS\ realization
 of the process. In this way, we can obtain a realization algorithm for \GBS{s}. 
 


==> JMLS_real_problem_formulation.tex <==
The terminology and notation used in this section 
is based on the conventions adopted in the literature, 
see \cite{CostaBook,Caines1}.
%
For the purposes of realization theory,
we will propose to look at stochastic
hybrid systems of a slightly more general form than
the one defined in \cite{CostaBook}.
A \emph{generalized
stochastic jump-linear systems, (GJLS)} is a 
system of the following form
%
\begin{equation}
\label{stoch_jump_lin:geq1}
H: 
\begin{cases}
   \x(t+1) & = ~ M_{\btheta(t+1),\btheta(t)}\x(t)+
   B_{\btheta(t+1), \btheta(t)}\v(t)  \\
   \y(t) &= ~ C_{\btheta(t)}\x(t) + D_{\btheta}\v(t)
  \mbox{ and }   \o(k) = \lambda(\btheta(k)) 
\end{cases} .
\end{equation}
\textbf{REMARK: Discuss the case of partialy observed discrete states}.
Here, the time-axis is assumed
to be the whole set of integers, i.e. 
$t \in \mathbb{Z}$.
%%or, in other words, $k$ is allowed
%%to be negative too. 
\begin{Remark}
Allowing negative time is a standard
practice in realization theory. The rational behind this
assumption is that one needs to take the infinite past
into the account. 
%%In this context, the state at time $t$
%%is just the projection (conditional expectation) of the
%%future outputs after time $t$ on the past outputs
%%up to time $t$. In order to formulate such a definition
%%formally, one needs to assume negative times as well.
\end{Remark}

 The stochastic processes 
 $\x$, $\btheta$, $\y$, and $\v$ are of the following form.
  The process $\btheta$ is called the \emph{discrete state process} and takes 
  values in the \emph{set of discrete states} $Q=\{1,2,\ldots, d\}$.
  The process $\x$ is called the \emph{continuous state process} 
  and takes values in one of the \emph{continuous-state spaces} 
  $\mathcal{X}_q=\mathbb{R}^{n_q}$, $q \in Q$. More precisely,
  for any time $t \in \mathbb{Z}$, the continuous
  state $\x(t)$ lives in the state-space component
  $\mathcal{X}_{\btheta(t)}$.
  The process $\y$ is the \emph{continuous output process} and takes
  values in the \emph{set of continuous outputs} $\mathbb{R}^{p}$.
  The process $\o$ is the \emph{discrete output process} and takes values in
   the \emph{set of discrete outputs} $O=\{1,2, \ldots, l\}$.
   Finally, the process $\v$ is the \emph{continuous noise} and takes
  values in $\mathbb{R}^{m}$.
  The map $\lambda: Q \rightarrow O$ is called the
  \emph{readout map} and it assigns a discrete output to
  each discrete state.
The matrices $M_{q_{1},q_{2}}$ are accordingly of the
form $M_{q_{1},q_{2}} \in \mathbb{R}^{n_{q_{1}} \times n_{q_{2}}}$
for any pair of discrete states $q_{1},q_{2} \in Q$.
The matrix $B_{q_{1},q_{2}}$ is of the form
$B_{q_{1},q_{2}} \in \mathbb{R}^{n_{q_{1}} \times m}$.
Finally, the matrix $C_{q}$ is of the form 
$C_{q} \in \mathbb{R}^{p \times n_{q}}$ for each discrete
state $q \in Q$. For each $q \in Q$, the matrix 
$D_{q}$ is a $p \times m$ matrix.
%%\begin{Remark}
%%For the sake of simplicity, here we assume that $D$
%%does not depend on the discrete state. If we allow
%%$D$ to depend on the discrete state, then we can
%%transform the jump-linear system to a jump-linear
%%system with the same discrete state and continuous
%%output but with $D=0$. We can achieve it by including
%%the noise $\v$ into the continuous state variable.
%%Hence, by considering only discrete st
%%\end{Remark}

We will make a number of assumptions on the stochastic
processes involved.
\begin{Assumption}
\label{Assumption0}
The discrete-state 
process $\btheta$ is a stationary finite-state  Markov process, 
with state-transition
probabilities 
$p_{i,j}=\Prob(\btheta(t+1)=i \mid \btheta(t)=j) > 0$ for
all $i,j \in Q$, moreover
the probability distribution
of the each discrete state $\btheta(t)$ is given by
the vector $\pi=(\pi_{1},\ldots, \pi_{d})^{T}$ where
$\pi_{i}=\Prob(\btheta(k)=i)$.
We assume  that the future discrete states
interact with past noises and continuous states only through
the past discrete states, and for any fixed sequence
of discrete states, the noise process is white and
the future noise and the current continuous
state are uncorrelated. 
In order to write these assumptions formally, 
denote by $\mathcal{D}_{t}$ the collection of
past discrete states $\btheta(t-k)$, $k \ge 0$, and
denote by $E[\z|\mathcal{D}_{t}]$
the conditional expectation of $z$ with respect to
$\mathcal{D}_{t}$. 
%%The assumptions above can be
%%written formally as follows
%%We will make the following assumptions on the
%%processes $\x$ and $\v$. 
We assume that for all $t \in \mathbb{Z}$, 
%%\begin{enumerate}
%%\item
   the collections of random variables
   $\{\x(t-l),\v(t-l), l \ge 0\}$ and
   $\{\btheta(t+l), l > 0 \}$
   are conditionally independent with respect to 
   $\mathcal{D}_{t}$, 
  %% for all $0 < $ are uncorrelated with
  %% with respect to $\mathcal{D}_{t}$, i.e. for
  %% all $0< l \le k$,
  %% $E[\x(t)\v(t+l)\btheta
%%\item
   for all $l > 0$
%%   $\v(t)$, $\v(t-l)$ are
   %%conditionally uncorrelated and zero mean with respect to 
   %%$\mathcal{D}_{t}$, i.e.
   $E[\v(t)\v(t-l)^{T}\mid \mathcal{D}_{t}]=0$ and
   %%and $\v(t)$ is conditionally zero mean, i.e.
   %%with respect to $\mathcal{D}_{t}$, that is,
   $E[\v(t) \mid \mathcal{D}_{t}]=0$, and
%%\item
   %%$\x(t)$ and $\v(t+l)$ are
   %%conditionally uncorrelated with respect to 
   %%$\mathcal{D}_{t+l}$, i.e.
   $E[\x(t)\v(t+l)\mid \mathcal{D}_{t+l}]=0$ for all $l \ge 0$.
%%\end{enumerate}
%%We will assume that $\v$ is a white noise process,
%%i.e. zero mean and the variables $\v(t)$ are uncorrelated.
%%Moreover, we we assume that $\btheta(t+l)$, and $\x(t)$ are
%%conditionally independent with respect to the
%%$\btheta(t)$
%%,\btheta(t-2),\ldots $ 
%%for all $t \in \mathbb{Z}$ and $l > 0$.
%%We assume that $\x(k)$ and
%%$\v(k)$ are uncorrelated for all $k \mathbb{Z}$. We also
%%assume that $\v(k)$ and $\chi(\btheta(t)=q)$ are uncorrelated
%%for all $k,t \in \mathbb{Z}$ and $q \in Q$, and
%%that $\v(t)$ and $\btheta(t+l)$ are conditionally independent
%%with respect to $\btheta(t)$ for all $t \in \mathbb{Z}$
%%and $l > 0$.
\end{Assumption}
%%that $\y(t)$ and $\btheta(t+l)$ 
%%are conditionally independent with respect to
%%The assumption above implies that
%%$\{ \y(t-k) \mid k \ge 0\}$ and
%%$\{ \btheta(t+k) \mid k > 0\}$ are 
%%conditionally independent with respect to $\mathcal{D}_{t}$.
%%$\btheta(t)$ for all $t \in \mathbb{Z}$, $l > 0$.
%%Moreover, we assume that for all $k \in \mathbb{Z}$
%%$\x(k)$ and $\btheta(k+1)$ are conditionally independent
%%with respect to $\btheta(k)$.
%% process and that the system.
%% Define the stochastic process 
%% \( \widetilde{\x}(k)=(\x^{T}(k)\chi(\btheta(k)=1), 
%%    \x^{T}(k)\chi(\btheta(k)=2), \ldots, 
%%    \x^{T}(k)\chi(\btheta(k)=d))^{T}
%% \)   
%% The it is easy to see that the following holds.
%%  \begin{equation}
%%  \label{stoch_jump_lin:eq1.1}
%%  \widetilde{H}: \left \{
%%  \begin{split}
%%   \widetilde{\x}(k+1) & = A_{\widetilde{\btheta}(k)}
%%   \widetilde{\x}(k)+B_{\widetilde{\btheta}(k)}\v(k)  \\
%%   \y(k) &= C_{\widetilde{\btheta}(k)}\widetilde{\x}(k) 
%%    \mbox{ and }   \o(k) = \widetilde{\lambda}(\widetilde{\btheta}(k)) 
%%  \end{split}
%%  \right. .
%%  \end{equation}
%% That is, the system $\widetilde{H}$ is  well-defined
%% stochastic jump-linear system of the form 
%% (\ref{stoch_jump_lin:eq1.1}) and it produces the same
%% output process as generalized stochastic jump-linear systems
%% $H$. The only restriction is that the transition
%% probability $p_{(q_{1},q_{2}),(q_{3},q_{4})}$
%% of the process $\widetilde{\btheta}$ is zero
%% for  all states such that $q_{2} \ne q_{4}$.
%%In order to be able to develope realization theory, we need
%%to make a number of assumption on the GJLS. These assumptions
%%render the continuous state and output processes wide-sense
%%stationary.
\begin{Assumption}
\label{Assumption1}
   The Markov process $\btheta$
   is stationary and ergodic, hence for all $q \in Q$, 
   $\sum_{s \in Q} p_{q,s}\pi_{s}=\pi_{q}$.
\end{Assumption}
\begin{Assumption}
\label{Assumption1.5}
  Let $n=n_{1}+n_{2}+\cdots + n_{d}$ and define the
  $n^{2} \times n^{2}$ matrix
  \begin{equation}
    \widetilde{M}=\begin{bmatrix}
                p_{1,1}M_{1,1} \otimes M_{1,1}^{T}  & 
		%%p_{1,2}M_{1,2} \otimes M_{1,2} & 
		\cdots &
		p_{1,d}M_{1,d} \otimes M_{1,d}^{T} \\
                p_{2,1}M_{2,1} \otimes M_{2,1}^{T} & 
		%%p_{2,2}M_{2,2} \otimes M_{2,2} & 
		\cdots &
		p_{2,d}M_{2,d} \otimes M_{2,d}^{T} \\
		\vdots & %%\vdots &
		\cdots & \vdots \\
                p_{d,1}M_{d,1} \otimes M_{d,1}^{T} &
		%%& p_{d,2}M_{d,2} \otimes M_{d,2} & 
		\cdots &
		p_{d,d}M_{d,d}  \otimes M_{d,d}^{T}. \\
		\end{bmatrix}	
  \end{equation}
 %% In order to render the processes $\x$ and $\y$ wide-sense
  %%stationary, we will require that 
  We will assume that
  $\widetilde{M}$ be \emph{stable}, that is,
  for any eigenvalue $\lambda$ of $\widetilde{M}$ we have $|\lambda| < 1$.
 \end{Assumption}
%% Assumption \ref{Assumption1} implies
 We get 
 the following
 result.
%% which is based on
 %%the well-known criteria
 %%for mean-square stability of jump-linear systems from
 %%condition on mean-square stability 
 %%\cite{CostaBook}.
  \begin{Lemma}
  \label{stoch_jump_stab:lemma1}
   If Assumption \ref{Assumption0} -- \ref{Assumption1.5} hold, then 
   there exists a unique collection of
   $n_{q}\times n_{q}$ matrices $P_{q}$ with
   $q \in Q$, such that $P_{q}$ satisfy
    \begin{equation}
 \label{stoch_jump_lin:eq2}
 P_{q}=\sum_{s \in Q} 
                     p_{q,s}M_{q,s}P_{s}M_{q,s}^{T}+B_{q,s}Q_{q,s}B_{q,s}^{T}, %%p_{q,s}\pi_{s},
  \end{equation}
  where $Q_{q,s}=E[\v(t)\v(t)^{T}\chi(\btheta(t+1)=q, \btheta(t)=s)]$.
  \end{Lemma}
\begin{Assumption}
\label{Assumption2}
   Assume that Assumption \ref{Assumption0} -- \ref{Assumption1.5} hold.
   Recall the definition of $\mathcal{D}_{t}$ from
   Assumption \ref{Assumption0}.
   Let $P_{q}$, $q \in Q$ be the unique collection of
   matrices satisfying (\ref{stoch_jump_lin:eq2}).
   We require that  for all $t \in \mathbb{Z}$, 
   $\x(t)$ is conditionally zero mean with respect to $\mathcal{D}_{t}$, 
   i.e.
   $E[\x(t) \mid \mathcal{D}_{t}]=0$, 
   and for all $q \in Q$,
   $E[\x(t)\x(t)^{T}\chi(\btheta(t)=q)]=P_{q}$ holds,
   where 
  $\chi$ denotes the indicator function, \ie $\chi(A)=1$ if the event $A$ is true, and 
  $\chi(A)=0$ otherwise.
 %% and the matrices 
   %%matrices $P_{q} \in \mathbb{R}^{n_{q} \times n_{q}}$, $q \in Q$
   %%satisfy
  \end{Assumption}
Assumptions \ref{Assumption1} and \ref{Assumption2}
are necessary in order to make the continuous state and
output process stationary. 
%%\begin{Remark}
%%\end{Remark} 
\begin{Remark} 
\label{gjmls:jmls}
Note that the classical definition of discrete-time 
jump-linear systems \cite{CostaBook} differs from
(\ref{stoch_jump_lin:geq1}). The main difference is that in
our framework the continuous state transition rule depends
not only on the current but also on the next discrete state.
The classical definition and (\ref{stoch_jump_lin:geq1}) are
equivalent in the following sense. A classical jump-linear
system also satisfies our definition. Conversely, a system
of the form (\ref{stoch_jump_lin:geq1}) can be rewritten
as a classical jump-linear system, with the same noise and
output processes, but with the discrete-state process
$\btheta$ replaced by
$\widetilde{\btheta}(t)=(\btheta(t+1),\btheta(t))$.
%%and the
%%continuous state process and the system matrices are replaced
%%by a continuous state process and system matrices living in
%%the continuous space $\mathbb{R}^{n_1+n_2+\cdots +n_d}$.
The reason that we choose to work with systems of the
form (\ref{stoch_jump_lin:geq1}) instead of classical
jump-linear system is the following. 
As it will be shown in this paper,
systems of the form (\ref{stoch_jump_lin:geq1}) 
admit a nice realization theory. However,
it is unclear whether one can also obtain such results
for classical jump-linear systems.
%%not succeed in getting such a characterization directly for
%%classical jump-linear systems. 
%%Since any GJMLS can be transformed
%%into a jump-linear system producing the same output processes,
%%identification and realization algorithms for GJML systems
%%can be combined with the transformation sketched above to
%%obtain classical jump-linear realizations.
\end{Remark}
%%\subsection{The Realization Problem for
%%                 Stochastic Jump-Linear Systems}
%%<<<<<<< cdc07-real.tex
%%\label{real:problem_form}		 
%%Recall the notion of \emph{weak and strong realization} for 
%%linear stochastic systems \cite{Caines1}. 
%%Below we will define what we mean by saying that a 
%%process is realized by a GJLS.
%%a similar concept for 
%%generalized stochastic jump-linear systems. 
%%Notice that in \cite{MPRV:HSCC} we already defined
%%=======
%%Recall the notion of \emph{weak and strong realization} for linear stochastic systems \cite{Caines1}. In this subsection, we will formulate a similar concept for stochastic jump-linear systems. In \cite{HSCC:MPRV} we already defined
%%>>>>>>> 1.5
%%the notion of realization of a classical 
%%stochastic jump-linear system.
%%and Remark \ref{gjmls:jmls}
%%provides a link between the definition of \cite{MPRV:HSCC}
%%and the definition below.
%%we have already noted that any GJLS can be transformed to
%%a classical stochastic jump-linear system with the
%%same continious and discrete output processes. Hence,
%%by saying that a GJLS is a weak respectively strong
%%realization of a process whenever the corresponding classical
%%stochastic jump-linear system is a weak (strong)
%%realization of the process already we already have
%%an adequate definition of the notion of realization.
%%Notice that in \cite{MPRV:HSCC} we already presented
%%necessary conditions for existence of a realization
%%by a stochastic jump-linear system. Due to 
%%Remark \ref{gjmls:jmls} these necessary conditions are
%%also necessary conditions for existence of a 
%%GJLS realization.
%%Since in this paper we present
%%sufficient conditions only when the discrete state is fully
%%observed, we will define what we mean by GJLS
%%realization only for this case.
%% 
  %%First of all,
  %%we will assume that the discrete state is fully observable,
  %%that is, $\widetilde{\o}=\btheta$ is a finite-state
  %%\begin{Definition}[Realization by GJLS]
  
  Below we will define the notion of a realization
  by a GJLS.
  Let $\widetilde{\y}$ be a zero-mean wide-sense
  stationary process with values in $\mathbb{R}^{p}$.
  %%Fix the set of discrete state $Q=\{1,\ldots, d\}$ 
  Fix a
  Markov-process $\btheta$ taking values in $Q=\{1,\ldots,d\}$ and
  defined on the time axis of all integers $\mathbb{Z}$.
 \begin{Definition}[Realization by GJMLS]
  Assume that $H$ is a  GJLS of the form
  (\ref{stoch_jump_lin:geq1}) and
  the discrete state process of $H$ is $\btheta$.
 %% and with the  
  %%discrete state process
  %%$\btheta$ 
  Then $H$
  is said to be a %%\emph{square-mean realization}
  or simply a \emph{realization} of $\widetilde{\y}$, 
   if
 the continuous output process $\y$ of $H$
 equals to $\widetilde{\y}$
 in the square-mean sense, that is, for any 
 time instant $k \in \mathbb{Z}$,
 $E[(\widetilde{\y}(k)-\y(k))^{T}(\widetilde{\y}(k)-\y(k))]=0$.
 \end{Definition}
 In the sequel we will keep the discrete state process
 $\btheta$ fixed and whenever we speak of
 a GJLS realization %%(weak or square-mean)
 of the process $\widetilde{\y}$, we
 will always mean a GJLS realization %%in the weak or
 %%square-mean sense 
 whose discrete state process is $\btheta$.
 
 It is easy to see that
 if $H$ is a square-mean realization of
 $\widetilde{\y}$, then  for all $t \in \mathbb{Z}$
 and for all $q_0,\ldots, q_k \in Q$, $k\ge 0$
  \begin{equation}
  \label{eq:stat}
  \begin{split}
   &  E[\widetilde{\y}(t+k)\widetilde{\y}(t)\chi(\btheta(t+i)=q_{i},i=0,\ldots, k)]= \\
   &  E[\y(k+t)\y(t)
     \chi(\btheta(i+t)=q_{i}, i=0,\ldots, k)]
 \end{split}    
 \end{equation} 
 That is, the fact that $H$ is a realization of
 $\widetilde{\y}$ imposes constraints on the second-order
 moments of $\widetilde{\y}$ described in (\ref{eq:stat}).
 If we recall the notion of a weak realization from
 \cite{MPRV:HSCC}, then it follows easily that
 if $H$ is a realization of $\widetilde{\y}$,
 then the classical stochastic jump-linear system
 corresponding to $H$ is a weak realization of
 $\widetilde{\y}$. In addition, we get the
 following.
 %%$H$ is also a weak realization of 
 %%$(\widetilde{\y})$.
 %%The fact that $H$
 %%is a weak-realization of the processes $(\widetilde{\y},\widetilde{\o})$
 %%imposes some constraints on the probability distribution of
 %%the processes $\widetilde{\o}$ and $\widetilde{\y}$. 
 %%If $H$ is a square-mean realization of 
 %%$\widetilde{\y}$, then it imposes a much
 %%stronger condition on $\widetilde{\y}$.
%%  such that for any $q_1,\ldots, q_{k} \in Q$,
  %%$k \ge 0$ the expectation
  %%$E[\widetilde{\y}(t+k-1)\widetilde{\y}(t)\chi(\btheta(t+i-1)=q_{i},i=1,\ldots, k\})$ is independent of $t$, i.e.
  %%for all $t \in \mathbb{Z}$.
%%Denote by $Q^{+}$ the set of all non-empty sequences
%%of elements of $Q$ and define the map
%%$\CD_{\btheta,\widetilde{\y}}:Q^{+} \rightarrow \mathbb{R}^{p \times p}$ by
%%\begin{equation}
%%\begin{split}
%%  \CD_{\btheta,\widetilde{\y}}(q_{0}q_{1}\cdots q_{k}) &=  \\
%%  & E[\widetilde{y}(k)\widetilde{\y}(0)^{T}
%%     \chi(\btheta(i)=q_{i}, i=0,\ldots,k)]. 
%%\end{split}
%%\end{equation}
%%If $\btheta$ is clear from the context, we will write
%%$\CD_{\widetilde{\y}}$ instead of $\CD_{\btheta,\widetilde{\y}}$.
%%Now we are readu to define the concept of weak 
%%realization by a GJMLS.
%%The map $\CD_{\btheta,\widetilde{\y}}$ gives the
%%covariance of $\widetilde{\y}(k)$ and 
%%$\widetilde{\y}(0)$, provided that the proces 
%%$\btheta$ takes values $q_{0},\ldots, q_{k}$ in the
%%first $k+1$ time instances. That is, 
%%$\CD_{\widetilde{\o},\widetilde{\y}}$ collects information on
%%the second-order moments of $\widetilde{\y}$.\footnote{
%%Notice the similarity between $\CD_{\widetilde{\o},\widetilde{\y}}$
%% and the generalized covariances in \cite{StochBilin}.}
%% 
%%Consider now a jump-linear system $H$ of
%%the form (\ref{stoch_jump_lin:eq1}) and
%%recall the definition of the processes 
%%$\y$ and $\o$. If \textbf{Assumption 1} and 
%%\textbf{Assumption 2} hold, then $\y$ is wide-sense stationary
%%and zero-mean and $\btheta$ is stationary. Hence, 
%%$\CD_{\btheta,\y}$ is well-defined. In fact,
%%they depend only on 
%%the matrices $M_{q_{1},q_{2}},B_{q_{1},q_{2}},C_{q_{1}}$, $q_{1},q_{2} \in Q$, the 
%%discrete state-transition probabilities $p_{q_{1},q_{2}}$,
%%$q_{1},q_{2} \in Q$, the probability
%%distribution $\pi$ of the discrete-state process. 
%%%%and the readout map $\lambda$.
%%To emphasize that $\CD_{\o,\y}$ depends only
%%on the parameters of $H$, we will denote $\CD_{\o,\y}$ by $\CD_{H}$.
%%  These maps are important, because they contain information
%%  about the probability distribution of the output processes
%%  generated by $H$. In fact, the following is true.
%% We will say that a zero-mean process $\z(t)$ with values in 
%% $\mathbb{R}^{m}$ is conditionally Gaussian with
%% respect to $\btheta$, if for all $t_1 < \ldots < t_{n}$
%% if the conditional distribution function
%% $\Prob(\z(t_1) \le x_1, \ldots, \z(t_{n}) \le x_{n} \mid \btheta(t), t \le t_n )$ is Gaussian.
  \begin{Proposition}
  If $\widetilde{\y}$ is a conditional Gaussian
  process with respect to the process $\btheta$, then 
  the second-order moments
  in the left-hand side of (\ref{eq:stat})
  uniquely determine the distribution of $\widetilde{\y}$.
  %%If $\y$ is the output of the system $H$ of
  %%the form (\ref{stoch_jump:lin:geq1}) and
  %%$\x$ is conditionally Gaussian with respect to
  %%$\btheta$ and $\v$ is Gaussian, then 
  %%$\y$ is conditionally Gaussian with respect to $\btheta$.
  In particular, if $H$ is a GJLS  realization
  of $\widetilde{\y}$, $H$ is of the form (\ref{stoch_jump_lin:geq1}), and both $\widetilde{\y}$ and $\y$
  are conditionally Gaussian with respect to $\btheta$,
  then the probability distributions of $\y$ and 
  $\widetilde{\y}$ are identical.
  \end{Proposition}
%%  We will say that a GJMLS $H$ is a 
%%  square mean 
%%  Markov-process with state-space
%%  We will call a GJMLS $H$ a \emph{square-mean
%%  realization}
%%  of $\widetilde{\y}$, if $H$ is a square-mean 
%%  realization
%%  of $(\widetilde{\y},\btheta)$ and the 
%%  discrete-state  process of $H$ 
%%  equals $\btheta=\widetilde{\o}$ and the readout map
%%  $\lambda$ is the identity
%%  map. By a minimal GJMLS realization  of $\widetilde{\y}$
%%  we will mean a GJMLS realization $H$ such that
%%  for any other GJMLS realization $H^{'}$ of $\widetilde{y}$
%%  it holds that 
%%  $\dim H \le \dim H^{'}$.
 %%Consider a stationary process $\widetilde{\o}$ taking values in the finite output 
%% space $O$, and a wide-sense stationary, zero-mean
%% stochastic process $\widetilde{\y}$ taking values in the continuous
%% output space $\mathbb{R}^{p}$. 
%% Let $O^{+}$ be the set of all nonempty words in $O$,
%%  i.e. $O^{+}=O^{*} \setminus \{\epsilon\}$.
 %%For all $o_{0},o_{1},\ldots, o_{k} \in O$, $k \ge 0$,
 %%define the  maps
 %%$\PD_{\widetilde{\o}}: O^{+} \rightarrow \mathbb{R}$ and 
 %%$\CD_{\widetilde{\o}, \widetilde{\y}}:O^{+} \rightarrow \mathbb{R}^{p \times p}$
% as follows
%% \begin{equation}
%% \begin{split} 
%%   \PD_{\widetilde{o}}(o_{0}o_{1}\cdots o_{k}) &=
%%     \Prob(\widetilde{\o}(i)=o_{i}, i=0,\ldots, k) \\
%%Notice that the map $\PD_{\widetilde{o}}$ gives the probability
%%distribution of the stochastic process $\widetilde{\o}$, while

%%The assumption that $Q=O$ is critical here. 
%%Intuitively, the more information about the discrete state 
%% is preserved by the discrete output, i.e. the closer $\o$ is
%% to $\btheta$, the better estimate of the probability distribution of
%% $\y$ is provided by $\CD_{H}$. 
%%With the notation above, we are now ready to define a notion of weak realization for stochastic jump-linear systems. 
%%\begin{Definition}[Weak Realization By GJMLS]
%%  A generalized stochastic-jump linear system $H$ 
%%  whose discrete state process is $\btheta$
%%  is said to be a \emph{weak stochastic realization of $\widetilde{\y}$}, if 
%% $\CD_{\btheta,\widetilde{\y}}=\CD_{H}$.
%% \end{Definition}
 %%Later in the paper we will show that if the whole discrete state is
 %%observable, then $(\widetilde{\y},\widetilde{\o})$ has a
 %%weak realization by a GJLS if and only if it has a 
 %%square-mean realization by a GJLS.
%%
%%We will
%%now show that  $(\widetilde{\y},\widetilde{\o})$
%%has a weak realization by a stochastic jump-linear system, 
%%only if certain families of formal power series are rational. 

Finally, we shall define the notion of a minimal
(weak or square-mean) realization by a GJLS system.
%%As we have already noted above, we assume that
%%the set of discrete state space of the systems involved
%%is fixed and is equal to $Q$ and the discrete state
%%process is fixed and it is equal to $\btheta$.
Define the \emph{dimension} of the GJLS $H$ as
\[ \dim H =n_{1}+n_{2}+\cdots+n_{d} \]
We call a realization $H$ of $\widetilde{\y}$
\emph{minimal}, whenever 
the dimension of $H$ is the smallest possible
among all those GJLS which are %%a weak or square-mean 
realizations of $\widetilde{\y}$.
\begin{Remark}
 Notice that two GJLSs can have the same dimension even
 if the dimensions of
 the individual continuous components are completely
 different.
%% For instances, two GJLS
 %%with continuous components of dimensions 
 %%$(3,2,2)$ and $(3,3,1)$  will have the same dimension
 %%$7$ according to our definition.
\end{Remark}


==> JMLS_real_stability_power_series.tex <==
Since our goal is to use formal power series to build a stochastic
realization theory for jump-linear systems,  we will need to restrict our attention to formal power series that are stable in some sense, similarly to the case of linear systems. In this subsection, we consider the notion of square summability for formal power series, and translate the requirement of square summability into algebraic properties of their representations.

More specifically, consider a formal power series $S \in \mathbb{R}^{p}\ll \Sigma^{*} \gg$ and define the sequence 
%
 \begin{align} 
 L_{n}=\sum_{k=0}^{n} \sum_{\sigma_{1} \in \Sigma} \cdots 
 \sum_{\sigma_{k} \in \Sigma} 
 ||S(\sigma_{1}\sigma_{2}\cdots \sigma_{k})||^{2}_{2} .
 \end{align}
%
where $||\cdot||_{2}$ is the Euclidean norm
in $\mathbb{R}^{p}$. 
The series $S$ will be called \emph{square summable}, if the
limit $\lim_{n \rightarrow +\infty} L_{n}$ exists and it
is finite. The family 
 $\Psi=\{ S_{j} \in \mathbb{R}^{p}\ll \Sigma^{*} \gg \mid j \in J\}$
 will be called \emph{square summable}, if
 for each $j \in J$, the formal power series 
 $S_{j}$ is square summable. 

We now characterize square summability of a family of formal power series in terms of the stability of its representation. Let $R=(\mathbb{R}^{n}, \{ A_{\sigma} \}_{\sigma \in \Sigma}, B,C)$ be an arbitrary representation of $\Psi=\{ S_{j} \in \mathbb{R}^{p}\ll \Sigma^{*} \gg \mid j \in J\}$.  Assume that
   $\Sigma=\{\sigma_{1},\ldots, \sigma_{d}\}$, where $d$ is the number of
   elements of $\Sigma$, 
%%  $d=card(\Sigma)$  
 and consider the matrix 
 \( \widetilde{A}=\sum_{i=1}^{d} A_{\sigma_{i}} \otimes A_{\sigma_{i}}^{T} \).
%%  \begin{align}
%%     \widetilde{A}_{R}=\begin{bmatrix}
%%                    A_{\sigma_{1}} \otimes A_{\sigma_{1}} & 
%%		    A_{\sigma_{2}} \otimes A_{\sigma_{2}} & \cdots & 
%%		    A_{\sigma_{d}} \otimes A_{\sigma_{d}}  \\
%%                    A_{\sigma_{1}} \otimes A_{\sigma_{1}} & 
%%		    A_{\sigma_{2}} \otimes A_{\sigma_{2}}  & \cdots & 
%%		    A_{\sigma_{d}} \otimes A_{\sigma_{d}} \\
%%                   \vdots     & \vdots    & \vdots & \vdots \\
%%                    A_{\sigma_{1}} \otimes A_{\sigma_{1}} & 
%%		    A_{\sigma_{2}} \otimes A_{\sigma_{2}} & \cdots & 
%%		    A_{\sigma_{d}} \otimes A_{\sigma_{d}} 
%%                  \end{bmatrix} \in \mathbb{R}^{n^{2}d \times n^{2}d},
%%  \end{align}
  where $\otimes$ denotes the Kronecker product.
  We will call $R$ \emph{stable}, if the matrix
  $\widetilde{A}$ is stable, i.e.
  %%complex $\lambda \in \mathrm{C}$ which lies outside or on the
  %%unit disk, i.e. for all $\lambda \in \mathrm{C}$
  %%with $|\lambda| \ge 1$.
  %%, \ie 
  if all
  its eigenvalues $\lambda$ lie inside the unit disk ($|\lambda| < 1$).
   We have the following.
 %% \begin{Lemma}
 %% \label{hscc_pow_stab:lemma1}
 %%  $R$ is stable if and only if for any $x \in \mathbb{R}^{n}$,
 %%  the formal power series $S(w)=A_{w}x$, $w \in \Sigma^{*}$
 %%  is square summable.
 %% \end{Lemma}
  \begin{Theorem}[\cite{MPRV:HSCC}]
  \label{hscc_pow_stab:theo2}
A rational family of formal power series is square summable if and only if all minimal representations are stable.
  \end{Theorem}
  
   Notice the analogy with the case of linear systems, where the minimal
   realization of a stable transfer matrix is also stable. 


%%\subsection{ $L_{q}$ Spaces of Sequences Indexed by
%% words over $\Sigma$ }
%% In what follows we will define $L_{q}$ spaces for 
%% sequences indexed with words 
%% over a fixed alphabet $\Sigma$ and
%% coefficients $\mathbb{R}^{n \times p}$. Let 
%% $L \subseteq \Sigma^{+}$ a set of nonempty words.
%%%% and
%% %%denote by $S(n,p,L)$ the set of all
%% %%functions of
%% %%the form $\alpha: L \rightarrow \mathbb{R}^{n \times p}$.
%% %%That is an element of $S(n,p,L)$ is
%% %%simply a sequence of $n \times p$ matrices
%% %%indexed by nonempty words. 
%% We will denote any $n \times p$ matrix values function
%% $\alpha: L \rightarrow \mathbb{R}^{n \times p}$
%% by $\alpha=[ \alpha(w) \mid w \in L]$. We will think 
%% of $f$ as an \emph{(possibly infinite) row vector indexed by elemennts of $L$}. In complete analogy with
%% the finite case, $f^{T}$ will denote the (possibly infinite)
%% \emph{column vector} 
%% $\alpha=[ \alpha^{T}(w) \mid w \in L]^{T}$.
%% of $p \times n$ matrices indexed by elements of $L$.
%% 
%% For 
%% each $0 < q < +\infty$ define the space $L_{q}(n,p, L)$
%% of all row vectors $\alpha=[\alpha(w) \mid w \in L]$ 
%% such that the following infinity series converges
%% \begin{equation}
%%	\sum_{w \in \Sigma^{+}} || \alpha(w) ||_{2}^{q} < +\infty
%% \end{equation}
%% where $||.||_{2}$ denotes the eucledian norm in $\mathbb{R}^{n \times p}$, i.e.
%% \( ||(p_{i,j})_{i=1,\ldots,n, j=1,\ldots,p}||_{2}=
%%    \sqrt{\sum_{i=1}^{n}\sum_{j=1}^{p} p_{i,j}^{2}}
%% \)   
%% It is easy to see that $L_{q}(n,p, L)$ is a linear space
%% and in fact it is a Banach space  for the norm
%% %%\begin{equation}
%% \(
%%  ||\alpha||_{q}=(\sum_{w \in \Sigma^{+}} ||\alpha(w)||_{2}^{q})^{1/q}
%% \). 
%% %%\end{equation}
%%%% In fact, the space $L_{q}$ can be obtained by applying the 
%%%% classical definition of $L_{q}$ spaces to the set of all
%%%% words over $\Sigma$ using the $\sigma$-algebra generated
%%%% by the set of all singleton sets and using the counting measure
%%%% $\mu$, i.e. the $\sigma$-algebra is generated by 
%%%% the sets $\{w\}$, for each word $w \in \Sigma^{+}$ and 
%%%% $\mu(\{w\}=1$ for each word $w \in \Sigma^{+}$.
%%%% In analogy with $l_{2}$ spaces, the space
%%%% $L_{2}(1,p,\Sigma^{+})$ is also a Hilbert-space with the
%%%% scalar product $<\alpha,\beta>=\sum_{w \in \Sigma^{+}} \alpha(w)\beta^{T}(w)$.
%%%% We define the $L_{\infty}(n,p,\Sigma^{+})$ space as the
%%%% linear space of all \emph{bounded formal power series},
%%%% i.e. $\alpha \in S(n,p,\Sigma^{+})$ belongs
%%%% to $L^{\infty}(n,p,\Sigma^{+})$ if and only if
%%%% there exists $M > 0$ such that
%%%% \begin{equation}
%%%%  \forall w \in \Sigma^{*}: ||\alpha(w)||_{2} \le M
%%%% \end{equation}
%% Notice that $L_{1}(n,p,L) \subseteq L_{q}(n,p,L)$
%%%% \subseteq L_{\infty}(n,p,\Sigma^{+})$ 
%% for all 
%% $0 < q < +\infty$.
%% Let $\bar{L}$ another subset of all nonempty words
%% $\Sigma^{+}$.
%% Consider a double indexed sequence 
%% $T=(T_{w,v})_{w\in L, v \in \bar{L}}$ of $p \times p$
%% matrices. Assume that there exists $M >0$ such that for
%% all $w \in L, \bar{w} \in \bar{L}$
%% \begin{equation}
%% \label{map:assump1}
%%  \sum_{v \in \bar{L}} ||T_{w,v}||_{2}^{2} < M 
%%  \mbox{ and }
%%  \sum_{v \in L} ||T_{v,\bar{w}}||_{2}^{2} < M
%% \end{equation}
%% where 
%% $||(P_{i,j})_{i,j=1,\ldots,p}||_{2}=\sqrt{\sum_{i=1}^{p}\sum_{j=1}^{p} P_{i,j}^{2}}$
%% is the eucledian norm on the $p\times p$ matrices.
%% That is, we assume that the sequence in 
%% (\ref{map:assump1}) is convergent and bounded by $M$ for all
%% words $w$ over $\Sigma$.
%% \begin{Proposition}
%% With this assumption
%%%% , using the discussion in
%%%% \cite{Balakrishnanm}, Chapter3, page 98, 
%% for any $n \ge 1$, $T$
%% defines uniquely a linear bounded
%% map $T:L_{1}(n,p,\bar{L}) \rightarrow L_{2}(n,p,L)$
%% defined as
%% \begin{equation}
%% \label{map:assump:def}
%%  T(\alpha)(w)=\sum_{v \in \bar{L}} \alpha(v)T_{v,w} 
%% \end{equation}
%% for each sequence $\alpha$ in the space 
%% $L_{1}(n,p,\bar{L})$. 
%% \end{Proposition}
%%%% \begin{proof}
%%%%  First, \( \sum_{v \in \Sigma^{+}, |v| \le n} ||\alpha(v) T_{v,w}||_{2} 
%%%%  \le \sum_{v \in \Sigma^{+}, |v| \le n}
%%%%       ||\alpha(v)||_{2}\cdot ||T_{v,w}||_{2} \le
%%%%       \sqrt(M) \cdots ||\alpha||_{1}
%%%%   \),
%%%%   hence the series in (\ref{map:assump:def}) is absolutely
%%%%   convergent, hence $T(\alpha)(w)$ is well-defined for
%%%%   each $w$.
%%%%   Second, assume for simplicty that $n=1$ and notice that 
%%%%   \(||\sum_{v \in \Sigma^{+}, |v| \le N} \alpha(v)T_{v,w})||^{2} 
%%%%      = \sum_{v,u \in \Sigma^{+}, |v|,|u| \le N}
%%%%        (\alpha(v)T_{v,w})(\alpha(u)T_{u,w})^{T} \le
%%%%	\sum_{v,u \in \Sigma^{+}, |u|,|v| \le N}
%%%%	|(\alpha(v)T_{v,w}T_{u,w}^{T}\alpha(u)|
%%%%	\le
%%%%	\sum_{v,u \in \Sigma^{+}, |v|,|u| \le N}
%%%%	||\alpha(v)||_{2}||\alpha(u)||_{2}
%%%%	\frac{1}{2}(||T_{v,w}||_{2}^{2}+||T_{u,w}||_{2}^{2})
%%%%   \)
%%%%   Hence, we get that 
%%%%   \( 
%%%%      \sum_{w \in \Sigma^{+}, |w| \le N}
%%%%      ||\sum_{v \in \Sigma^{+}, |v| \le N} \alpha(v)T_{v,w}||^{2}
%%%%      \le 
%%%%      \sum_{v,u \in \Sigma^{+}, |u|,|v| \le N} 
%%%%      ||\alpha(v)||_{2} ||\alpha(u)||_{2}
%%%%      \sum_{w \in \Sigma^{+}, |w| \le N}
%%%%      \frac{1}{2}(||T_{v,w}||_{2}^{2}+||T_{u,w}||_{2}^{2})
%%%%      \le M \sum_{v,u \in \Sigma^{+}, |u|,|v| \le N}
%%%%      ||\alpha(v)||_{2} ||\alpha(u)||_{2} \le
%%%%      M \cdot ||\alpha||_{1}
%%%%   \)
%%%%   which implies that $\alpha T$ belongs to
%%%%   $L_{2}(1,p,\Sigma^{+})$. The proof of $n > 1$ uses the fact
%%%%   that 
%%%%   \( ||\sum_{w \in \Sigma^{+}} \alpha(w)T_{w,v}||^{2}_{2}=
%%%%      \sum_{i=1}^{n} ||\sum_{w \in \Sigma^{+}} \alpha_{i}(w)T_{w,v}||_{2}^{2}
%%%%    \) 
%%%%    where $\alpha_{i}(w)$ denotes the $i$th row of $\alpha(w)$.
%%%% \end{proof}
%% Following our view of $\alpha$ as
%% a row vector, we will denote $T(\alpha)$ by $\alpha T$.
%% Assume that $L=\bar{L}$, i.e. the map
%% $T$ maps from $L_1(1,p,L)$ to $L_2(1,p,L)$.
%% We will call $T$ \emph{symmetric} if
%% $T_{w,v}=(T_{v,w})^{T}$. 
%% We will say that $T$ is 
%% \emph{strictly positive definite}, if 
%% for all nonzero $\alpha \in L_{1}(1,p,L)$
%% \begin{equation}
%% \label{map:posdef:def}
%%  0  < \sum_{w,v \in L} \alpha(w)T_{w,v}\alpha^{T}(v)
%% \end{equation}
%% It is easy to see that if $T$ is strictly positive definite,
%% then for any $N > 0$ the finite matrix
%% $(T_{w,v})_{w,v \in L, |w|,|v| < N}$ is strictly
%% positive definite.
%%%%         \sum_{v \in \Sigma^{+}}
%%%%	 || \sum_{w \in \Sigma^{+}} \alpha_{i}T_{w,v}||_{2}
%%%%	 ||\alpha(v)||_{2}
%%%%      \le ||\alpha T||_{\infty} ||\alpha ||_{1} 
%%%%  \), which implies    
%%%%  $||\alpha T||_{\infty} > p ||\alpha|_{1}$, which
%%%%  by Theorem 4.15, Chapter 4, page 97 \cite{RudinFunc}
%%%%  together with $T=T^{*}$
%%%%  implies that $T$ is bijective.
%%%%  If $\alpha \in L_{1}(n,p,\Sigma^{+})$, then 
%%%%  $\beta = T \alpha$, if and only if
%%%%  $\beta_{i}=T\alpha_{i}$, $i=1,\ldots,n$, where 
%%%%  $\alpha_{i}$, $\beta_{i}$ stands for the sequence formed
%%%%  by the $i$th  rows of elements of $\alpha$ and $\beta$.
%%%%  Hence, if $T$ is bijective as a map 
%%%%  $T:L_{1}(1,p,\Sigma^{+}) \rightarrow L_{\infty}(1,p,\Sigma^{+})$
%%%%  then it is bijective as a map 
%%%%  $T:L_{1}(n,p,\Sigma^{+}) \rightarrow L_{\infty}(n,p,\Sigma^{+})$.
%%%% \end{proof}
%% 
%%\section{ A Generalized Bilinear Stochastic 
%%             Realization Problem and Its Solution }
%%  In this section we will formulate a linear filtering
%%  problem and we will present its solution. The problem
%%  generalizes the classical Kalman-filtering/realization
%%  problem. Its solution provides a solution to the
%%  bilinear stochastic realization problem \cite{StochBilin}
%%  and will be shown to provide a solution to the
%%  realization problem for GJLS. 
%%
%%\subsection{ Hilbert spaces of square integrable random
%%           variables }
%%\label{hilb:rand}	   
%%  Denote by $L_{2}$ the Hilbert-space of square integrable
%%  $0$-mean random variables.
%%  That is, a random
%%  variable $x$  belongs to $L_{2}$, 
%%  whenever
%%  $E[x]=0$ and the square-mean $E[xx]$ exists.
%%  Then for
%%  any $x,y$ in $L_{2}$ the cross-corellation 
%%  $E[xy^{T}]$ is well defined. Moreover, 
%%  $<x,y>=E[xy]$ defines a scalar product on 
%%  $L_{2}$. We can also define a norm
%%  $||x||=sqrt(E[xx^{T}])$. If we identify every two
%%  random variable $x,y$ for which 
%%  $E[(x-y)(x-y)]=0$, then $L_{2}$ will become a Hilbert-space
%%  with the scalar product and norm above.
%%  If $x$ and $y$ are two scalar valued zero mean
%%  square-integrable random variables and
%%  $E[(x-y)(x-y)]=0$, then we will say that
%%  \textbf{$x=y$ ($x$ equals $y$) in the square-mean sense}.
%%  We will say that two vector valued random
%%  variables are \textbf{equal in the square mean sense},
%%  if the corresponding scalar components are equal
%%  in the square mean sense.
%%  If $y$ is a $\mathbb{R}^{p}$ valued random variable
%%  such that $y=(y_{1},\ldots, y_{p})^{T}$, i.e.
%%  $y_{i}$, $i=1,\ldots,p$ are the scalar valued
%%  components of $y$. By abuse of terminology, we will
%%  say that $y$ belongs to $L_{2}$ if each of the
%%  component $y_{i}$ belongs to $L_{2}$.
%%  If $Z$ is a subset of $\mathbb{R}^{p}$ valued
%%  random variables belonging to $L_{2}$, then denote
%%  by $\bar{\SPAN}\{z \mid z \in Z\}$ the closure of
%%  the linear subspace of $L_{2}$ spanned by the 
%%  scalar valued components of elements of $Z$.
%%  
%%  $E[y \mid Z]$ is the unique $p$-tuple 
%%  $(x_{1},\ldots,x_{p})^{T}$ of elements of $L_{2}$ such
%%  that for any element $x_{i}$, $i=1,\ldots, p$
%%  \begin{enumerate}
%%  \item
%%  \label{orth:cond1}
%%     $x_{i} \in \bar{\SPAN}\{ z \mid z \in Z \}$
%%  \item
%%   \label{orth:cond2}  
%%     $y_{i}-x_{i}$ is orthogonal to $Z$, or,
%%     equivalently, $E[(y_{i}-x_{i})z^{T}]=0$ for
%%     all $z \in z$.
%%  \end{enumerate}
%%  $E[y \mid Z]=(x_{1},\ldots, x_{p})^{T}$ 
%%  is unique is square mean, that is,
%%  for any tuple $\hat{h}=(\hat{x}_{1},\ldots, \hat{x}_{2})$
%%  which satisfies Condition \ref{orth:cond1} and
%%  \ref{orth:cond2}, it holds that 
%%  $E[(x_{i}-\hat{x}_{i})^{2}]=0$, $i=1,\ldots, p$, i.e.
%%  \begin{equation}
%%  E[(E[y \mid Z]-\hat{h})(E[y \mid Z]-\hat{h})^{T})]=0
%%  \end{equation}

